Guided Image Restoration via Simultaneous Feature and Image Guided Fusion

Guided image restoration (GIR), such as guided depth map super-resolution and pan-sharpening, aims to enhance a target image using guidance information from another image of the same scene. Currently, joint image filtering-inspired deep learning-based methods represent the state-of-the-art for GIR tasks. Those methods either deal with GIR in an end-to-end way by elaborately designing filtering-oriented deep neural network (DNN) modules, focusing on the feature-level fusion of inputs; or explicitly making use of the traditional joint filtering mechanism by parameterizing filtering coefficients with DNNs, working on image-level fusion. The former ones are good at recovering contextual information but tend to lose fine-grained details, while the latter ones can better retain textual information but might lead to content distortions. In this work, to inherit the advantages of both methodologies while mitigating their limitations, we proposed a Simultaneous Feature and Image Guided Fusion (SFIGF) network, that simultaneously considers feature and image-level guided fusion following the guided filter (GF) mechanism. In the feature domain, we connect the cross-attention (CA) with GF, and propose a GF-inspired CA module for better feature-level fusion; in the image domain, we fully explore the GF mechanism and design GF-like structure for better image-level fusion. Since guided fusion is implemented in both feature and image domains, the proposed SFIGF is expected to faithfully reconstruct both contextual and textual information from sources and thus lead to better GIR results. We apply SFIGF to 4 typical GIR tasks, and experimental results on these tasks demonstrate its effectiveness and general availability.

==> sec_bak/0_abstract.tex <==
\begin{abstract}
Guided image restoration (GIR) aims to enhance a target image using guidance information from another image of the same scene.
Filtering-based DNN methods have achieved SOTA performance by using DNNs to learn parameters in joint filters or modeling joint image filtering mechanisms into guided restoration networks.
However, these methods still suffer from over-transferred artifacts or loss of details because of insufficient exploration of correlations of physical mechanisms with DL algorithms or inadequate intergradation of the physical fusion principles within their frameworks.
To simultaneously inherit the strength of joint filters and DNN, we proposed a Guided Filter (GF) inspired fusion block to combine sources in the image domain. What's more, to mitigate the previous problems, we further explore the relatives between GF mechanisms and the effective cross-attention (CA) module and build a guided fusion module with the proposed GF-inspired CA (GICA) module for the feature-level fusion. Both the image-level and feature-level restoration results are integrated for a satisfactory final output with rich details and outstanding perceptual performance.
Finally, we conduct extensive experiments on several GIR benchmarks and show that our proposed Guided Image Restoration Network (GIRNet) presents SOTA performance on these specific tasks and has generalization ability for the GIR problem.
\end{abstract}

==> sec_bak/1_intro.tex <==
\section{Introduction}
With the rapid development of photography techniques, images can be captured from multiple sensors simultaneously under the same scene. Consequently, we can expect higher quality imaging by making use of rich and complementary information delivered by those multi-modal source images. Considering the case with two source images, one may be interested in restoring one of these two images with the guide information transferred from the other one \cite{he2010guided, he2012guided}, which can be referred to as guided image restoration (GIR), including guided denoising \cite{dong2022abandoning}, super-resolution \cite{yang2017pannet, hui2016depth} and enhancement \cite{xiong2021mffnet}. This type of tasks has attracted increasing research interest in recent years due to its wide applications in remote sensing \cite{cheng2016survey}, auto driving \cite{liao2020dvi}, computational photography \cite{petschnigg2004digital}, etc. 
% The main goal of GIR tasks is to restore a high-quality composite image with rich details by incorporating structural information from a guidance image into the target image. A key challenge is how to effectively transfer textual cues from the guidance image while reducing redundant information. 
% This aims to preserve contextual information present in both images while removing artifacts, thus enhancing the quality of the filtered output image.

% The GIR methods can mainly be divided into two categories, which are model-driven approaches and data-driven approaches. 
{\color{red}Traditionally, the GIR problem is mainly solved by various joint image filters, including Bilateral Filter (BF) \cite{tomasi1998bilateral}, Guided Filter (GF) \cite{he2010guided}, and their variants \cite{he2012guided, xiao2012fast}.
Such joint filters exploit complementary information across source images by transferring extracted textual contents from one input (guidance) to enhance another target image (filtering input).
However, these methods highly rely on the manually designed filtering mechanism, which may not be flexible enough to adapt to complex image structures, and thus the performance is still limited.}

In the last decade, motivated by their success in wide applications, deep learning methods have been introduced to deal with the GIR tasks. A straightforward way along this line is to directly feed the input source images to a deep neural network (DNN), and output the restoration result in an end-to-end way \cite{li2016djif,deng2020cunet,kim2021deformable}. Observing that well-designed DNNs are effective feature extractors, such a strategy realizes image fusion at the feature level. Another way of using DNN for GIR is to explicitly take the traditional joint filtering mechanism into consideration, and learn components of filters by DNNs \cite{wu2018fgf, pan2019spatially}. Such methods directly perform GIR in the image, or pixel level, which inherits the advantage of joint filtering, while being more flexible. Thanks to the powerful learning ability, both types of deep learning methods are expected to perform well on a specified GIR task after proper training.
% With the development of deep-learning algorithms, deep-learning-based models have produced more satisfactory fusion results.
% In the beginning, researchers directly fed features extracted from source images with sub-networks to a unified fusion network for restoration \cite{deng2020cunet, xu2020fusiondn}. However, these approaches failed to further explore intrinsic correlations between sources, leading to incomplete structure preservation and artifact removal. Considering this, some researchers attempted to find solutions from traditional methods, whose has shown effectiveness in detail reconstruction. One of the most direct ways is to transform computed parameters of joint filters into learnable ones.
% For example, Wu et al. \cite{wu2018fgf} proposed an end-to-end Guided Filter by replacing mean operators with convolution blocks. 
% Pan et al. \cite{pan2019spatially} proposed to input the source images into a unified network to jointly learn the parameters of GF in an end-to-end manner.
% % Zhong et al. \cite{zhong2021dagif} used learned adaptive filter kernels instead of traditional artificial ones for fusion. 
% On the contrary, some other researchers \cite{li2016djif, kim2021deformable} got rid of the filter framework and designed individual guidance, filtering, and fusion networks to simulate joint image filtering.  

\begin{figure}[t]
	\centering
	\setlength{\abovecaptionskip}{0.1cm}
        \includegraphics[width=1\linewidth]{./results/Intro_v2.pdf}
	\caption{Visualization of present filtering-inspired methods.}
	\vspace{-0.5cm}
	\label{fig:intro} 
\end{figure}

% Leveraging the instructive nature of joint filtering mechanisms, both of these methods have achieved outstanding performance on image restoration tasks that incorporate side information or guidance.
However, these deep-learning approaches still have their own limitations.
In specific, the former strategy which mainly implements feature-level fusion, though good at restoring the contextual information of images, e.g., removing noise, may lose fine-grained textual information, such as edges, delivered by the guide image.
On the contrary, the latter methodology can do better in transferring the textual information from the guidance to the target at the feature level but tends to result in more unexpected distortions of image contents.
% The former ones tend to closely follow the original design of joint image filters, only replacing parts of the filter with CNN layers and implementing fusion in the image domain. While this helps preserve structural and textural information, the restoration capability is limited because of the weak ability to restore the degraded contents. 
% The latter ones tend to rely on the network's learning ability with high degrees of freedom and only apply filtering and fusion in the feature domain, yet the results inevitably suffer from information loss as the network flexibility is enhanced.
These can be more intuitively observed by the guided depth map super-resolution (GDSR) example as shown in Fig.\ref{fig:intro}.
It can be seen from Fig. \ref{fig:intro} that the results of CU-Net \cite{deng2020cunet} and  FDKN \cite{kim2021deformable}, which belong to the former type methods, look smoother, but the edges are somewhat blurry. In comparison, the FGF \cite{wu2018fgf} and SVLRM \cite{pan2019spatially} transfer more textual information from the guide RGB image, but lead to unnatural distortions in contents, such as ghost effects. These observations motivate us to leverage the benefits of both deep methodologies while mitigating their current limitations, seeking for better GIR performance.
% GF and its extended deep learning-based methods, which strictly adhere to the hand-crafted transformation mechanism in the image domain, tend to transfer structural details excessively. Consequently, the results demonstrate images with unexpected artifacts, commonly referred to as ghosting effects and over-transferred structures, due to over-reliance on manually designed operations in the spatial domain. In contrast, FDKN \cite{kim2021deformable} and DAGF \cite{zhong2021dagif}, which eschewed physical filtering models in favor of utilizing neural networks to directly simulate fusion processes directly within feature spaces, may be susceptible to losing fine-grained textural details and generating over-smoothed outcomes due to the intrinsic properties of DL-based information aggregation.




% However, early works focused on predicting the parameters of filters or replacing some operators in the filters with convolutional operators. Although these methods compared to traditional methods achieved improvements, due to the limited degrees of freedom and network scales, they were still unable to generate satisfactory filtering results.
% Some recent works have abandoned these constraints and tried to learn new adaptive filtering kernels. With this process, they can fully integrate the complementary information from both sources. While this approach can achieve relatively favorable results for tasks with salient guidance maps, in line with kernel prediction methods, it incurs higher memory demands at equivalent parameter scales; meanwhile, convolving solely with guidance maps neglects the significant role of the target image in the fusion problem (such as providing color and contextual information).

% {\textbf{To leverage the benefits of these approaches while mitigating their current limitations for enhanced fusion performance, }}
In this work, we propose a new DNN framework, called \textbf{Guided Image Restoration Network} (GIRNet), for the GIR tasks.
The proposed GIRNet combines the advantages of both of the aforementioned methodologies in using DNNs, by considering guided fusion operations simultaneously in image and feature domains. 
Specifically, in the image domain, GIRNet explicitly fuses input source images with the guided filtering \cite{he2010guided} fashion with key parameters predicted by specifically designed network modules, sharing the similar idea of FGF \cite{wu2018fgf} and SVLRM \cite{pan2019spatially};
% {\color{red} in the feature domain, GIRNet modifies the efficient transformer structures, or more concretely the cross-attention (CA) modules, facilitating a more effective guided fusion for the features extracted from different source images.Interestingly, the modified CA module can be seen as a generalization of the guided filtering mechanism, while implemented in the feature domain.}
{\color{red}in the feature domain, we propose a GF-inspired cross-attention (GICA) module, which integrates fusion mechanisms of GF with efficient transformer structures, concretely the cross-attention (CA) module, to facilitate a more effective guided fusion module for the features extracted from different source images. Furthermore, the GICA module can be seen as a generalization of the guided filtering mechanism, while implemented in the feature domain.}
The guided fusion outputs from image and feature domains are then aggregated for the final GIR result. 
Since the final result is contributed from both image and feature domains, it is expected to recover as much as possible textual information transferred from the guide image, while also faithfully restoring the contextual information from source images. 
% The proposed GIRNet mainly consists of three key modules: the semi-coupled multi-scale feature extraction (SMFE) module for feature representation; 
% the Image-Guided Fusion (ImGF) module, which enhances detail preservation by fusing two source images related to the low-light RAW one in the image domain; 
% and the Feature-Guided Fusion (FeGF) module, which extends the guided restoration to the feature domain in a multi-scale way to better combine the complementary information and reconstruct the degraded contents underlying the features extracted from different sources. 
% Notably, in the FeGF module, considering the limited ability to capture long-range dependencies of CNN layers, which are still used as the backbone in GIR tasks,
% we propose neighbor-cross-attention blocks for further improvement. 

Our \textbf{contributions} can be summarized as follows:
\begin{itemize}
\item {\color{red}We explored the connection between CA and guided filtering, and proposed the GICA module, which integrates the fusion principles of GA with the CA structure. Based on the GICA module, we designed a feature-guided fusion (FeGF) module to fuse multi-scale features extracted from source images. The FeGF module on the one hand can better capture the spatial dependencies due to CA operation, and on the other hand, can better fuse the complementary information from sources by virtue of the guided filtering mechanism.}

\item We designed an image-guided fusion (ImGF) module for image level fusion, which inherits the idea of learnable GF \cite{he2010guided}, but with modifications to make it more coincides with GF; and also a semi-coupled multi-scale feature extraction (SMFE) module based on the NAF blocks \cite{chen2022nafnet} for cooperatively extracting features from source images. Together with the FeGF module, we constructed the GIRNet for GIR tasks, which is expected to leverage the advantages of both methodologies discussed before.


\item  We applied the proposed GIRNet to for typical GIR tasks, including  guided depth image super-resolution, pan-sharpening, multi-frame image fusion (MFIF), and guided low-light raw image enhancement.
Extensive experiments on those tasks validate the effectiveness of GIRNet and demonstrate its wide applicability.
%Additionally, the generalization of our approach was evaluated on the tasks of low-light raw image enhancement (LIRE) and guided LRIE, demonstrating the efficacy of the proposed network for diverse data formats and single image restoration applications. A variety of formats and restoration scenarios were covered to validate that our method is effective across different GIR domains both qualitatively and quantitatively.
% The numeric and visualized results demonstrate that our proposed network outperforms other state-of-the-art methods both qualitatively and quantitatively. 
\end{itemize}

\begin{figure*}[t]
	\setlength{\abovecaptionskip}{0.2cm}
	\centering
	% \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
	\includegraphics[width=1\linewidth]{./network/GIRNet_v4.pdf}
	%\vspace{-0.5cm}
	\caption{The overview of GIRNet. The SMFE, ImGF, and FeGF modules are introduced in Section \ref{sec:smfe}, \ref{sec:imgf}, and \ref{sec:fegf}, respectively. $F_A$ and $F_B$ are convolutional layers to infer $A_{Im}$ and $B_{Im}$.}
	\label{fig:girnet}
	\vspace{-0.5cm}
\end{figure*}
%-------------------------------------------------------------------------
% \subsection{Language}

% All manuscripts must be in English.

% \subsection{Dual submission}

% Please refer to the author guidelines on the \confName\ \confYear\ web page for a
% discussion of the policy on dual submissions.

% \subsection{Paper length}
% Papers, excluding the references section, must be no longer than eight pages in length.
% The references section will not be included in the page count, and there is no limit on the length of the references section.
% For example, a paper of eight pages with two pages of references would have a total length of 10 pages.
% {\bf There will be no extra page charges for \confName\ \confYear.}

% Overlength papers will simply not be reviewed.
% This includes papers where the margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
% Note that this \LaTeX\ guide already sets figure captions and references in a smaller font.
% The reason such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts.
% The reviewing process cannot determine the suitability of the paper for presentation in eight pages if it is reviewed in eleven.

% %-------------------------------------------------------------------------
% \subsection{The ruler}
% The \LaTeX\ style defines a printed ruler which should be present in the version submitted for review.
% The ruler is provided in order that reviewers may comment on particular lines in the paper without circumlocution.
% If you are preparing a document using a non-\LaTeX\ document preparation system, please arrange for an equivalent ruler to appear on the final output pages.
% The presence or absence of the ruler should not change the appearance of any other content on the page.
% The camera-ready copy should not contain a ruler.
% (\LaTeX\ users may use options of \texttt{cvpr.sty} to switch between different versions.)

% Reviewers:
% note that the ruler measurements do not align well with lines in the paper --- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly.
% Just use fractional references (\eg, this line is $087.5$), although in most cases one would expect that the approximate location will be adequate.


% \subsection{Paper ID}
% Make sure that the Paper ID from the submission system is visible in the version submitted for review (replacing the ``*****'' you see in this document).
% If you are using the \LaTeX\ template, \textbf{make sure to update paper ID in the appropriate place in the tex file}.


% \subsection{Mathematics}

% Please number all of your sections and displayed equations as in these examples:
% \begin{equation}
%   E = m\cdot c^2
%   \label{eq:important}
% \end{equation}
% and
% \begin{equation}
%   v = a\cdot t.
%   \label{eq:also-important}
% \end{equation}
% It is important for readers to be able to refer to any particular equation.
% Just because you did not refer to it in the text does not mean some future reader might not need to refer to it.
% It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3 column 1''.
% (Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
% All authors will benefit from reading Mermin's description of how to write mathematics:
% \url{http://www.pamitc.org/documents/mermin.pdf}.

% \subsection{Blind review}

% Many authors misunderstand the concept of anonymizing for blind review.
% Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

% Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
% That is all.
% (But see below for tech reports.)

% Saying ``this builds on the work of Lucy Smith [1]'' does not say that you are Lucy Smith;
% it says that you are building on her work.
% If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

% An example of a bad paper just asking to be rejected:
% \begin{quote}
% \begin{center}
%     An analysis of the frobnicatable foo filter.
% \end{center}

%    In this paper we present a performance analysis of our previous paper [1], and show it to be inferior to all previously known methods.
%    Why the previous paper was accepted without this analysis is beyond me.

%    [1] Removed for blind review
% \end{quote}


% An example of an acceptable paper:
% \begin{quote}
% \begin{center}
%      An analysis of the frobnicatable foo filter.
% \end{center}

%    In this paper we present a performance analysis of the  paper of Smith \etal [1], and show it to be inferior to all previously known methods.
%    Why the previous paper was accepted without this analysis is beyond me.

%    [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
% \end{quote}

% If you are making a submission to another conference at the same time, which covers similar or overlapping material, you may need to refer to that submission in order to explain the differences, just as you would if you had previously published related work.
% In such cases, include the anonymized parallel submission~\cite{Authors14} as supplemental material and cite it as
% \begin{quote}
% [1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324, Supplied as supplemental material {\tt fg324.pdf}.
% \end{quote}

% Finally, you may feel you need to tell the reader that more details can be found elsewhere, and refer them to a technical report.
% For conference submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a tech report for further details.
% Thus, you may say in the body of the paper ``further details may be found in~\cite{Authors14b}''.
% Then submit the tech report as supplemental material.
% Again, you may not assume the reviewers will read this material.

% Sometimes your paper is about a problem which you tested using a tool that is widely known to be restricted to a single institution.
% For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the 1970 audience would like to hear about your
% solution.
% The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

% You can handle this paper like any other.
% Do not write ``We show how to improve our previous work [Anonymous, 1968].
% This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
% That would be silly, and would immediately identify the authors.
% Instead write the following:
% \begin{quotation}
% \noindent
%    We describe a system for zero-g frobnication.
%    This system is new because it handles the following cases:
%    A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
%    Ours handles it by including a foo term in the bar integral.

%    ...

%    The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
%    It displayed the following behaviours, which show how well we solved cases A and B: ...
% \end{quotation}
% As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
% A reviewer might think it likely that the new paper was written by Zeus \etal, but cannot make any decision based on that guess.
% He or she would have to be sure that no other authors could have been contracted to solve problem B.
% \medskip

% \noindent
% FAQ\medskip\\
% {\bf Q:} Are acknowledgements OK?\\
% {\bf A:} No.  Leave them for the final copy.\medskip\\
% {\bf Q:} How do I cite my results reported in open challenges?
% {\bf A:} To conform with the double-blind review policy, you can report results of other challenge participants together with your results in your paper.
% For your results, however, you should not identify yourself and should not mention your participation in the challenge.
% Instead present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison to other results.\medskip\\

% \begin{figure}[t]
%   \centering
%   \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
%    %\includegraphics[width=0.8\linewidth]{egfigure.eps}

%    \caption{Example of caption.
%    It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
%    \label{fig:onecol}
% \end{figure}

% \subsection{Miscellaneous}

% \noindent
% Compare the following:\\
% \begin{tabular}{ll}
%  \verb'$conf_a$' &  $conf_a$ \\
%  \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
% \end{tabular}\\
% See The \TeX book, p165.

% The space after \eg, meaning ``for example'', should not be a sentence-ending space.
% So \eg is correct, {\em e.g.} is not.
% The provided \verb'\eg' macro takes care of this.

% When citing a multi-author paper, you may save space by using ``et alia'', shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word).
% If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
% However, use it only when there are three or more authors.
% Thus, the following is correct:
%    ``Frobnication has been trendy lately.
%    It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
%    Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

% This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has just two authors.

% \begin{figure*}
%   \centering
%   \begin{subfigure}{0.68\linewidth}
%     \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
%     \caption{An example of a subfigure.}
%     \label{fig:short-a}
%   \end{subfigure}
%   \hfill
%   \begin{subfigure}{0.28\linewidth}
%     \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
%     \caption{Another example of a subfigure.}
%     \label{fig:short-b}
%   \end{subfigure}
%   \caption{Example of a short caption, which should be centered.}
%   \label{fig:short}
% \end{figure*}


==> sec_bak/2_relatedwork.tex <==
\section{Related Work}
\subsection{Traditional guided image restoration methods}
% Traditional approaches for addressing guided image restoration problems primarily rely on constructing joint image filters.
Traditionally, GIR tasks can be addressed by joint image filtering, where the filtering is implemented on the to-be-restored image, while coefficients of the filter are computed by also considering the guidance image. Many joint image filters were designed to achieve this goal, such as the bilateral filter \cite{tomasi1998bilateral}, guided filter \cite{he2010guided, he2012guided} and their variants \cite{li2014weighted, xiao2012fast}.
% {\color{red} Another methodology to deal with GIR tasks is to formulate the problem within an optimization model, which minimizes an objective function constructed according to the concerned task. For example, Aodha et al.\cite{mac2012patch} employed random field models to solve the GDSR problem, and Wang et al. \cite{wang2018bayesian} reformulated the pan-sharpening task as a variational optimization model method to solve the problem.} 
{\color{red} Another type of methodology to deal with GIR tasks is to formulate an optimization model for a specific problem, such as the construction of a Markov random field labeling problem for GDSR \cite{mac2012patch} and the introduction of a variational optimization model for pan-sharpening \cite{wang2018bayesian}.}
% The data fidelity term ensures that the filtered output is close to the target image, while the regularisation term encourages the output to exhibit structural similarities to the guidance image. 
% The efficacy of joint image filters has been demonstrated in computer vision problems, with such approaches continuing to see widespread application in both image fusion \cite{ShutaoLiImageFusion2013, bavirisetti2017medicalfusion} and segmentation \cite{zhang2022segmentation} to the present day.
Comparing the two methodologies, the latter is more task-specific, while the former is more general and has wider applications{\color{red} \cite{he2012guided, li2014weighted, tomasi1998bilateral}}.
However, these methods highly rely on manually designed filters or optimization models, and thus the performance is still limited.

\subsection{DL-based guided image restoration methods}
Motivated by their success in other applications, especially in image restoration tasks, deep learning methods have dominated the GIR tasks in recent years.
% \noindent \textbf{Filter-based methods} 

Since joint image filtering takes an important position in traditional GIR methods, many deep learning methods were constructed to try to improve it or motivated by it.
Among them, several works attempted to improve upon GF by replacing average operators with convolution layers for a learnable GF \cite{wu2018fgf} or learning GF parameters end-to-end \cite{pan2019spatially}. 
% For example, Wu et al.\cite{wu2018fgf} proposed to replace average operators with convolution layers for a learnable GF; Pan et al. \cite{pan2019spatially} took a step further by learning GF parameters end-to-end rather than relying on fixed formulas.
Though reasonable and efficient, such methods may suffer from limited performance, since they overly reinforce the mechanisms of joint filters in the image level and thus constrain the freedom and learning ability of powerful deep neural networks, leading to unsatisfied results with over-transferred artifacts.

Other than those methods that try to make filters learnable in the image domain, most researchers resorted to further designing filters-oriented yet effective network architectures for better performance in the feature domain. 
\cite{li2016djif, li2019joint} proposed to use CNN-based sub-networks to split common and salient features from sources for final fusion results.
\cite{Su_2019_pac, kim2021deformable, zhong2021dagif} built filtering-inspired networks with deformable convolution for adaptive filtering location \cite{kim2021deformable} or predictable kernels with learnable weights \cite{zhong2021dagif, Su_2019_pac}.  
% Deng et al. \cite{deng2020cunet} proposed a CNN network based on a novel multi-modal convolutional sparse coding (MCSC) model to split the common features from the unique features between the source images. 
% % Beyond GF, other approaches also sought to advance this methodology. 
% Li et al. \cite{li2016djif, li2019joint} proposed to construct CNN-based networks for selectively transferring salient structures that are consistent with source images.
% Su et al.\cite{Su_2019_pac} proposed a pixel-adaptive convolution operation, which is a simple yet effective modification of standard convolutions, for better guided restoration performance.
% Kim et al. \cite{kim2021deformable} proposed a CNN-based framework yet learned both kernel weights and sampling locations with deformable convolution layers.
% Zhong et al. \cite{zhong2021dagif} aimed to obtain adaptive kernels to fully leverage complementary details across source images.

% Xu et al. \cite{xu2020fusiondn} propose a Dense-Block-based network \cite{huang2017densenet} to automatically estimate the importance of source image contents, determining adaptive preservation degrees for information, and use continual learning \cite{lee2017overcoming} to unsupervisedly solve multiple fusion tasks.
% Zhao et al. \cite{zhao2023cddfuse} proposed a two-stage unsupervised training approach wherein they incorporate the Restormer architecture \cite{zamir2022restormer} within an embedding module to learn representations from unlabeled data.
% \vspace{-0.5cm}

However, some researchers pointed out that the performance of the aforementioned methods is still limited due to the lack of elucidation of an explicit and well-founded physical model. 
To mitigate this issue, algorithm unrolling methods \cite{deng2019deep, madunet} have been developed for GIR tasks. Except for the mentioned model-inspired methods, effective multi-modal fusion networks are also designed in supervised \cite{deng2020cunet} and unsupervised way\cite{xu2020fusiondn,zhao2023cddfuse}.
% Deng et al. \cite{deng2019deep} proposed to simultaneously learn three dictionaries and two transform matrices to combine the modalities of iterative shrinkage and thresholding algorithm (ISTA) and turned the model into a deep neural network in an unrolling way.
% Zhou et al. \cite{madunet} presented an unrolling network by a maximal a posteriori (MAP) estimation model employing a dual-prior formulation for super-resolution.
% However, the inherent algorithmic complexity demands relatively more computational resources and longer reference time. 

% \subsection{Guided image restoration tasks}
% Other than the general-purpose GIR methods reviewed above, there are also many studies dealing with specific tasks. 
% Here, we briefly review several typical GIR tasks, that will be considered in our applications, and representative methods for those tasks.

% \noindent\textbf{Guided depth map super-resolution (GDSR)} 
% The goal of guided depth map super-resolution (GDSR) is to reconstruct a high-resolution (HR) depth map from a low-resolution (LR) depth input with the assistance of an HR RGB image captured of the same scene. 
% Traditional methods of GDSR can be categorized as filter-based and optimization-based. Filter-based methods utilize edge-preserving filters like BF \cite{tomasi1998bilateral, yang_2007_depth}, GF \cite{he2010guided, he2012guided}, and Static and Dynamic Filter \cite{Ham_2017_sd} to propagate depth boundaries from guidance images. 
% Optimization-based approaches formulate depth super-resolution as an energy minimization problem to model inter-dependencies between color and depth domains using techniques such as Markov random fields \cite{diebel2005application}, non-local means \cite{park2011high}, and total generalized variation regularization \cite{ferstl2013image}. 

% Recent deep-learning methods have achieved more advanced performance in this field. The filter-based generalized methods \cite{li2016djif, kim2021deformable,zhong2021dagif} have been applied to this task for guidance information transformation. Beyond them, other model-based methods have also achieved superior performance. For example, Zhao et al. \cite{zhao2022dct} introduced a Discrete Cosine Transform (DCT) module to reconstruct the multi-channel HR depth features; Lutio et al. \cite{de2022graphsr} utilized the implicit function theorem to infer an affinity graph to leverage complementary information from the source images.
% There are also many studies focusing on designing powerful network architectures. Hui et al. \cite{hui2016depth} introduced multi-scale guidance for hierarchical restoration. Guo et al. \cite{guo2018hierarchical} also built a multi-scale architecture yet further learned coarse-to-fine residual information to achieve the final HR depth map. 
% Zhong et al. \cite{zhong2021high} proposed an attention-based hierarchical multi-modal fusion network to effectively extract and combine relevant information.
% He et.al \cite{he2021towards} proposed to adaptively decompose high-frequency components from the RGB image to guide the depth map SR.
% % Lutio et al. \cite{de2022graphsr} built a differentiable optimization layer that operates on a learned affinity graph to leverage contextual and textual information from the source images. 
% Metzger et al. \cite{metzger2023guided} proposed to embed guided anisotropic diffusion into a CNN network to 
% combine the strengths of optimization-based and deep learning-based super-resolution. Zhao et al.\cite{zhao2023spherical} utilized Restormer-based encoders to extract features from source images and mapped them to a spherical space for better separation and alignment of private and shared information.







% \noindent\textbf{Pan-sharpening}
% Pan-sharpening aims to reconstruct an HR multi-spectral image (HRMS) from an LR multi-spectral image (LRMS) with the guidance of a panchromatic image (PAN).
% Conventional pan-sharpening methods are involved in component substitution (CS)-based \cite{carper1990use, chavez1991comparison, kwarteng1989extracting}, multi-resolution analysis (MRA)-based \cite{vivone2014multiresolution, alparone2016spatial, zheng2008remote}, and variational optimization (VO)-based \cite{he2014new, palsson2013new, fasbender2008bayesian, zhang2009noise}, and traditional machine-learning-based, which consists of dictionary learning \cite{zhu2012sparse}, compressive sensing techniques \cite{li2010new}, and image filtering \cite{liao2015two}.

% Compared to the traditional ones, deep-learning methods have achieved state-of-the-art performance. Except for the generalized filter-based methods \cite{pan2019spatially,wu2018fgf}, other specialized model-based methods have shown outstanding performance. Xu et.al \cite{xu2021gppnn} modeled the degradation model and introduced the unrolling algorithm. Zhou et.al \cite{madunet} further explored the unrolling-based way and embedded traditional priors to explicitly model the inner relationship between source images.
% Zhu et al. \cite{zhu2023probability} modeled the problem from a probabilistic perspective to explicitly utilize global information and built a new probabilistic-based block to improve the previous methods. 
% The others realized information fusion of the pan and multi-spectral image by concatenating both of the source images and inputting them into a sophisticatedly-designed network, based on convolution layers \cite{yang2017pannet} or self-attention blocks \cite{liang2022pmacnet}.

% \noindent\textbf{Multi-focus image fusion (MFIF) \label{sec:rlmff}}
% Multi-focus image fusion refers to a framework for synthesizing an all-in-focus output image by integrating spatially complementary visual content from multiple source frames exhibiting focus disparities. 
% Different from the above two GIR tasks, which have clear guidance, the MFIF can be considered a mutually guided restoration problem.
% Traditional MFIF methods can mainly be categorized into two classes, which are Transformation domain-based ones and Spatial domain-based ones. 
% Transformation domain methods perform manipulations in the transformation domain, such as discrete cosine transformation (DCT) \cite{phamila2013low}, discrete wavelet transformation (DWT) \cite{li1995multisensor}, and Non-subsampled contourlet transform (NSCT) \cite{yang2007image}.
% Spatial domain algorithms can be further divided into block-based or pixel-based ones. Block-based methods \cite{li2001combination} mainly calculated activity measures for blocks.
% % Pixel-based approaches provide more accurate focus/defocus classification and finer-grained maps by estimating measures directly on pixels.
% Pixel-based techniques include filter-based ones\cite{he2010guided, li2013image}, focus maps with boundary-based segmentation \cite{zhang2017boundary}, dense SIFT \cite{liu2015multi}, and matting-based activity measures \cite{li2013imagematting, chen2017robust}.

% For deep-learning methods, researchers have explored deeply both in supervised and unsupervised ways. Within the supervised way, Liu et al. \cite{liu2017multi} first introduced the CNN network for this task. Zhao et al. \cite{zhao2018multi} developed a multi-scale architecture for better feature extraction and fusion performance. 
% Compared with the supervised fashion, the unsupervised way might be of more interest, since the ground-truth images are generally difficult to obtain due to the focusing mechanism in the camera.  Among them, Densefuse \cite{li2018densefuse} and SESF \cite{ma2021sesf} used pre-trained autoencoders for feature extraction and fusion in high dimensions. MFFGAN \cite{zhang2021mffgan} introduced a GAN framework with constraints to generate fused images without labels. SMFuse \cite{ma2021smfuse} self-supervisedly trained a mask generator for focus maps. U2fusion \cite{xu2020fusiondn} embedded continual learning \cite{de2021continual} into DenseNet \cite{huang2017densenet}, achieving promising single-task results. SwinFusion \cite{ma2022swinfusion} proposed a cross-domain long-distance Swin Transformer for spatial feature extraction and fusion.
% % Pixel methods avoid blocky issues while enabling more localized focus estimation over entire images.


% \noindent \textbf{Guided Low-light RAW image enhancement (LRIE) \label{rw:lrie}}

% The LRIE task aims at enhancing the quality of the RAW image captured under extremely low-light conditions. The pioneering work was done by Chen et al. \cite{chen2018learning}, who built the SID dataset for DL-based training, and proposed a deep ISP pipeline with U-Net \cite{ronneberger2015u} which directly outputs clean normal-light sRGB images in an end-to-end way.
% % On the basis of the SID dataset and the proposed pipeline, multiple deep-learning methods{\color{red} \cite{chen2018learning, gu2019sgn, xu2020lrde, zhu2020eemefn} }for LRIE have been developed and achieved distinguished performance. Among these methods, a major clue for network design is to use the guided fusion mechanism, with either self-generated guidance or an auxiliary one.
% % {\color{red} For example, Gu et al. \cite{gu2019sgn} adopted a top-down self-guidance architecture to better exploit multi-scale features; 
% % % Xu et al. \cite{xu2020lrde} proposed a frequency-based decomposition and enhancement structure for sufficient noise removal; 
% % Zhu et al. \cite{zhu2020eemefn} generated multi-exposure frames from raw sensor images in order to fuse them for higher contrast, and utilized a pre-trained edge detection network for better detail preserving.}
% % %Since the noise contained in low-light RAW images is very complicated, Wei et al. \cite{wei2020eld} built a physical noise model, called ELD, to synthesize realistic noisy RAW images under extreme low-light conditions. This ELD noise model was latter adopted by Lu and Jung \cite{lu2022progressive} to synthesize data for adapting part of their proposed network to new camera models. 
% % % \noindent\textbf{Low-light Image Enhancement with additional guidance} 
% Considering the wide integration of multi-sensors in modern camera devices, LRIE with guidance has also been explored very recently. For example, white \cite{xia2021flash} or red flashlight \cite{xiong2021mffnet} was considered as the guidance for enhancing sRGB images, as well as the utilization of the infrared and near-infrared sensors \cite{jin2022darkvisionnet}; and monochrome images captured without the Bayer filter \cite{dong2022abandoning} were used for RAW images. Due to the auxiliary information provided by the guidance, especially the structural details, better-enhancing results can be expected.
% % {\color{red} This is because the LRIE problem is a complex task, including denoising, detail preservation, and image signal processing. Decomposing the problem by extracting multimodal source images and fusing them facilitates image restoration.}
% % \subsection{Pan sharpening}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




==> sec_bak/3_girnet.tex <==
\section{Guided Image Restoration Network}
Before presenting our GIRNet, we need to first review GF and CA, and then explore the connection between them to motivate our work. 
\subsection{Preliminaries}
\subsubsection{Guided Filter \label{sec:gf}}
GF \cite{he2010guided, he2012guided} is a versatile image processing tool, originally designed for filtering an input image with a guidance image.
Due to its ability to effectively fuse two source images via making use of complementary information delivered by them, GF has been applied to a variety of image processing tasks since being raised, including image fusion \cite{ShutaoLiImageFusion2013, bavirisetti2017medicalfusion} and image segmentation \cite{zhang2022segmentation}.
% It has since proven to be a powerful tool for various image processing tasks, such as image fusion \cite{ShutaoLiImageFusion2013, bavirisetti2017medicalfusion} and image segmentation \cite{zhang2022segmentation}.
The key assumption under GF is that the filtering output $Q$ is a linear transform of the guidance image $I$ in a window $\omega_{k}$ centered at the pixel $k$:
\begin{equation}
	Q_{j} = a_{k}I_{j} + b_{k},~~~ \forall j\in\omega_{k},
	\label{eq:1}
\end{equation}
% To determine the linear coefficients, we seek a solution to (3) that minimizes the difference between q and the filter input p. Specifically, we minimize the following cost function in the window:
where $a_{k}$ and $b_{k}$ are the constant coefficients of pixels in the window $\omega_{k}$, and the subscript $j$ refers to the $j$th pixel in $\omega_k$. The coefficients can be obtained by minimizing the following cost function within the window $\omega_k$: 
\begin{equation}
	E(a_k, b_k) = \sum\nolimits_{j \in \omega_{k}}{((a_k I_j + b_k - P_j)^2 + \epsilon a_k^2)},
	\label{eq:2}
\end{equation}
which ensures that the output $Q$ should also be close to input $P$. Here, $\epsilon$ is a regularization parameter preventing $a_{k}$ from being too large. The solution can be analytically computed:
\begin{gather}
	a_k = \frac{\frac{1}{|\omega|}\sum_{j\in\omega_{k}}{I_j P_j-\mu_k\bar{P}_k}}{\sigma_k^2 + \epsilon} = \frac{{\mathrm{Cov}(I,P)}_{k}}{\sigma_k^2 + \epsilon}, \label{eq:a_gf}\\
	b_k = \bar{P}_k -a_k\mu_k. \label{eq:b_gf}
\end{gather}
Here, $\mu_k$ and $\sigma_k^2$ are the mean and variance of $I$ in $\omega_{k}$, $|\omega|$ is the number of pixels in $\omega_k$, $\bar{P}_k=\frac{1}{|\omega|}\sum_{j\in\omega_{k}}{P_j}$ is the mean of $P$ in $\omega_k$ and $\mathrm{Cov}(\cdot,\cdot)_k$ indicates the covariance. Then the filtering output can be finally calculated by:
%\begin{align}
%	q_i &= \frac{1}{|\omega|} \sum_{k:i\in\omega_k}{(a_k I_i+b_k)}\label{eq:5}\\
%	&=\bar{a}_i I_i +\bar{b}_i,
%	\label{eq:6}
%\end{align}
\begin{equation}
	Q_j = \frac{1}{|\omega|} \sum\nolimits_{k:j\in\omega_k}{(a_k I_j+b_k)}=\bar{a}_j I_j +\bar{b}_j,
	\label{eq:6}
\end{equation}
where $\bar{a}_j = \frac{1}{|\omega|}\sum_{k\in\omega_{j}}{a_k} $ and $\bar{b}_j = \frac{1}{|\omega|}\sum_{k\in\omega_{j}}{b_k} $ by averaging all the possible values of $Q_j$ involved in all windows that contain $j$. Using matrix form, Eq. \eqref{eq:6} can also be written as
\begin{equation}
	Q_{GF}=A_{GF}\circ I+B_{GF},
	\label{eq:GF_matrix}
\end{equation}
where $A_{GF}$ and $B_{GF}$ are composed of $\bar{a}_i$s and $\bar{b}_i$s, respectively, and $\circ$ denotes the element-wise multiplication.
It can be seen that $A_{GF}$ explicitly depicts the correlation between the inputs $I$ and $P$ due to the covariance included in Eq.\ref{eq:a_gf}. {\color{red}Its effects can be more intuitively observed in Fig. \ref{fig:iabq}, that the calculated $A_{GF}$ reflects the structural information in $I$ that is related to $P$.}

\subsubsection{Cross-attention in DNNs \label{sec:ca}}
% The self-attention module has excelled at capturing intra-modal dependencies \cite{vaswani2017attention}, while it still limited in modeling multi-modal (or just multi-sequence) inter-source interactions. 
% Cross-attention \cite{tan2019lxmert} generalizes attention mechanisms through cross-domain querying, enabling representations from one sequence to attend to information encoded in another, and its effectiveness have been proved in various vision tasks, including classification \cite{chen2021crossvit}, segmentation \cite{ke2021prototypical}, compressive sensing \cite{song2023optimization}, and so on.
% Specifically, cross-attention permits values and keys originating from one modality to interact with keys originating from an alternate domain.
Recently, Transformers \cite{vaswani2017attention} have become dominant DNN architectures in various tasks \cite{liang2021swinir, khan2022transformers}. One of the key components of Transformers is the attention mechanisms \cite{mnih2014recurrent, vaswani2017attention}. Initially,  the self-attention module has been used to effectively capture dependencies within individual modalities or sequences 
% as demonstrated in \cite{vaswani2017attention}, its capabilities remain limited when modeling complex interactions between multiple sources of information. 
To model complex interaction between multiple sources, cross-attention (CA)\cite{vaswani2017attention, tan2019lxmert} was proposed to generalize the attention mechanisms through cross-domain queries. 
This cross-modal attention has shown success in various applications, including image classification \cite{chen2021crossvit}, image semantic segmentation \cite{zhang2022segmentation}, and compressive sensing \cite{song2023optimization}.

Mathematically, for patch tokens $x, y \in \mathbb{R}^C$, the cross-attention attention mechanism can be expressed as:
\begin{gather}
    Q_x=xW_q,
    K_y=yW_k,
    V_y=yW_v,\\ 
    A(x,y) = Softmax(\frac{Q_xK_y^T}{\sqrt{d}}), \label{eq:a}\\
    CA(x,y)= A(x,y)V_y
    =Softmax(\frac{Q_xK_y^T}{\sqrt{d}})V_y, \label{eq:cross}
\end{gather}
where $W_q, W_k, W_v \in \mathbb{R}^{C\times d}$ are learnable parameters, $C$ and $d$ are the token dimension and the scaling parameter.  
{\color{red}In this way, CA permits querying relationships between queries originating from one representation space and keys and values encoded in an alternative space, enabling more robust encoding of interdependencies across different informational sequences. Besides, to avoid vanishing gradients in deep networks, CA is always implemented with skip connects by adding the input $y$ before being outputted.}

\noindent \textbf{Dicussions.}
% It should be noticed that $A(\cdot, \cdot)$ in Eq.\ref{eq:a} attempted to depict the internal relation between input sources, and acquire finally acquire the attention map about one of the inputs, as shown in Eq.\ref{eq:cross}. 
% The purpose and implementation approach is similar to GF, and this inspires us to introduce the cross-attention module for more reasonable fusion architectures because it's reasonable and effective. 
% Section \ref{sec:gf} has demonstrated the utility of modeling inter-source relationships in guided image restoration tasks. The GF framework utilizes an attention mechanism, denoted $A_{GF}$ in Eq.
% \ref{eq:a_gf} to capture the inherent relations between different input sources. Specifically, as shown in Eq.
% \ref{eq:GF_matrix}, this attention mapping derives a weighted representation of the guidance $I$ based on its relationships to the filtering input $P$.
% The cross-attention module takes a similar approach, seeking to learn input interactions for more informed fusion. Specifically, we observe similarities in goals and methodology to GF, which aims to jointly attend to inputs to construct modal representations. In that, we propose extending GF's insights by introducing a cross-attention module to explicitly model dependencies of cross-modal features.
% Preliminary researchers exploring this approach have proved it to be a reasonable and effective design choice for Information interaction and fusion. Therefore, cross-attention can serve as a promising avenue for advancing research at GIR tasks.
Though looks very different at first glance, the GF and CA indeed share some similar mechanisms. Specifically, if we treat $x$ and $y$ in CA as $P$ and $I$ in GF, respectively, we can see from Eq. \ref{eq:cross} that the calculation of $A(x, y)$ is very similar to the calculation of $A_{GF}$, both of which are trying to capture the correlations between inputs. Besides, the $V_y$ term is indeed a transformation of $y$. Therefore, the overall process of CA, i.e., $A(x,y)V_y$ can be regarded as a kind of generalization of the $A_{GF}*I$ term in GF. The only intrinsic difference between GF and CA is the $B_{GF}$ term, which can in some sense be seen as the residuals from $P$, by eliminating the information correlated to $I$.
{\color{red}Since GF has been shown to be effective in fusing source images at the image level, while CA is powerful in feature level information fusion, the above observations of the connection between them motivate us to integrate them to build and introduce a 
GF-inspired cross-attention (GICA) block which is specific for GIR tasks (details are provided in Section. \ref{sec:fegf}) to DNN architecture, seeking for a better feature level fusion for the GIR tasks. In addition, we want to maintain the GF mechanism at the image level, inheriting similar ideas from previous studies \cite{alparone2016spatial,wu2018fgf}, which, together with the feature level fusion, constitutes the architecture of the proposed GIRNet.}

% From the equations mentioned above, 
% \subsection{Motivation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
	\setlength{\abovecaptionskip}{0.2cm}
	\centering
	% \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
	\includegraphics[width=1\linewidth]{./network/smfe_v2.pdf}
	%\vspace{-0.5cm}
	\caption{The overview of the SMFE Module. The details are introduced in Sec.\ref{sec:smfe}. NAF refers to the NAF-block proposed in \cite{chen2022nafnet}.}
	\label{fig:smfe}
	\vspace{-0.5cm}
\end{figure}


\subsection{Proposed Approach}
Now we are ready to discuss the details of the proposed GIRNet. In the following, we first discuss the overall structure and workflow of GIRNet and then provide details for each building block.
\subsubsection{Overall network structure and workflow}
Our proposed GIRNet comprises three key modules: a Semi-coupled Multi-scale Feature Extraction (SMFE) module for extracting multi-scale features from different sources, an ImGF module for image-level fusion, and a FeGF module for feature-level fusion. \textbf{In particular, the ImGF module is mainly designed to better preserve original details of source images by the explicit GF mechanism, while the FeGF module mainly contributes to better recovering contextual and textual information from diverse types of degradations by the proposed GICA operation, }%and correcting contextual information, 
as in Section \ref{sec:ablation}.
The overall network structure is shown in Figure \ref{fig:girnet}.

% \noindent \textbf{Workflow.}
Given the to-be restored image $P$ and the guidance image $I$ as input resources, GIRNet outputs $Q_{Out}$.
First, $P$ and $I$ are inputs to the SMFE module to jointly extract their multi-scale features. The extracted features are then passed to the ImGF and FeGF modules for subsequent processing. In the ImGF module, the extracted features, together with the input source images, are used to infer $A_{Im}$ and $B_{Im}$ for the guided fusion result $Q_{Im}$ in the image level. In the FeGF module, the extracted multi-scale features are first fused by GICA blocks at each scale and then aggregated by upsample blocks to obtain the final feature $q_{Fe}$. Finally, $Q_{Im}$ and $q_{Fe}$ are concatenated, and input to a small network with attention and convolutional layers to obtain the restored result $Q_{Out}$.
% The $L_1$ loss between $Q_{Out}$ and the ground truth $Q_{GT}$ is adopted for network training.

\subsubsection{Semi-coupled Multi-scale Feature Extraction (SMFE) module\label{sec:smfe}}
GIRNet first needs to extract features from the guidance image $I$ and the filtering input $P$. Rather than proposing them by two separate subnetworks, or simply concatenating as input to a single network, we introduce a coupled feature extraction module based on NAF-Block \cite{chen2022nafnet}, a simple yet effective image restoration tasks,  to jointly extract features from $I$ and $P$.
This module is expected to effectively capture the correlations between two source The detailed structure of SMFE is shown in Figure. \ref{fig:smfe}. As shown in the figure, we first initialize features of $I$ and $P$ as follows: 
\begin{gather}
    i_0 = GELU(Conv(I)), \\
    p_0 = GELU(Conv(P)),\\
    ip_0 = GELU(Conv(Cat(I,P))),
\end{gather}
where $Cat(\cdot,\cdot)$ denotes the catenating operation, $Conv(\cdot)$ refers to convolutional layers, and $GELU(\cdot)$ refers to the Gaussian Error Linear Unit (GELU) activation function \cite{hendrycks2016gaussian}. 
Then we build hierarchical architectures for multi-scale feature extraction as follows:
\begin{gather}
    i_{t+1} = (NAF(Cat(i_t, ip_t))+i_t)\downarrow,\\
    p_{t+1} = (NAF(Cat(p_t, ip_t))+p_t)\downarrow,\\
    ip_{t+1} = GELU(Conv(Cat(i_t, p_t)))\downarrow,
\end{gather}
where $t$ refers to the scale number ranging from integer 0 to 3, $NAF(\cdot)$ is the NAF-block in NAFNet \cite{chen2022nafnet}, and $(\cdot)\downarrow$ denotes convolutional layers with an average pooling operator for downsampling.
The multi-scale structure here can not only save computational cost but also facilitate better feature representation or both convolution and CA-based architectures, as claimed in \cite{chen2021crossvit}. 
With the above design, the feature extractor is expected to extract shared and private informative features effectively from input image pairs.
% Multi-scale feature representations have a long history in computer vision (e.g., image pyramids [1], scale-space representation [29], and coarse-to-fine approaches [28]). In the context of CNNs, multi-scale feature representations have been used for detection and recognition of objects at multiple scales [4, 22, 44, 26], as well as to speed up neural networks in Big-Little Net [5] and OctNet [6]. bLVNet-TAM [12] uses a two-branch multiresolution architecture while learning temporal dependencies across frames. SlowFast Networks [13] rely on a similar two-branch model, but each branch encodes different frame rates, as opposed to frames with different spatial resolutions. While multi-scale features have shown to benefit CNNs, it’s applicability for vision transformer still remains as a novel and largely under-addressed problem.

% \begin{figure}[t]
% 	\setlength{\abovecaptionskip}{0.2cm}
% 	\centering
% 	% \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
% 	\includegraphics[width=1\linewidth]{./results/IABQ.pdf}
% 	%\vspace{-0.5cm}
% 	\caption{Visualizations of $As$,$Bs$ with inputs and outputs of GF\cite{he2010guided} and the ImGF module of GIRNet.}
% 	\label{fig:iabq}
% 	\vspace{-0.5cm}
% \end{figure}

\subsubsection{FeGF module for feature-domain guided fusion \label{sec:fegf}}
% We also need an effective fusion module in the feature domain to address various degradation issues of multiple guided restoration tasks for better restoration results.
% As discussed in {\color{red} Section.\ref{sec:ca}}, we want to introduce CA to feature-level fusion, with modifications to let it follow the GF mechanism, aiming at a better-guided restoration.
{\color{red} As discussed in {\color{red} Section.\ref{sec:ca}}, we propose a GICA module that integrates the principles of GF and CA and want to introduce it to the feature-level fusion, aiming at a better-guided restoration.}

The detailed structure of the whole FeGF module is illustrated in Fig. \ref{fig:fegf}.
% As shown in Fig.\ref{fig:smfe} and introduced before, the inputs of the FeGF module are multi-scale features, including $i_ts$ and $p_ts$, extracted from the SMFE module, and the aim is to reconstruct feature maps from degradations in the feature domain.
As shown in Fig. \ref{fig:fegf}, the FeGF module consists of four GICA blocks for fusing the multi-scale features extracted by the SMFE module. In each scale, the GICA block fuses features in the following way:
\begin{gather}
    q_t = CA(i_t, p_t)+b_t,\label{eq:fegf_ca}\\
    b_t = SA(LN(Cat(i_t, p_t))) + p_t,
\end{gather}
where $LN(\cdot)$ refers to layer normalization, and $SA(\cdot)$ is the self-attention block processing and follows:
\begin{gather}
    Q_z = zW_q,
    K_z = zW_k,
    V_z = zW_v,\\
    A(z) = Softmax(\frac{Q_zK_z^T}{\sqrt{d}}), \label{eq:a}\\
    SA(z)= A(z)V_z
    =Softmax(\frac{Q_zK_z^T}{\sqrt{d}})V_z,  
\end{gather}
{ \color{red} As can be seen from Eq.\ref{eq:fegf_ca}, we replace the original a skip-connect term $p_t$ with a "residual" term $b_t$ to compute the fusion result $q_t$ in addition to CA.} According to the discussions in Section III-A3, the calculation of $q_t$ can be seen as a generalization of GF, which inherits the intrinsic mechanism of GF, while is expected to be more flexible for feature fusion. 
Besides, the calculation of $b_t$ in Eq. \ref{eq:fegf_ca} also follows the principle of computing $B_{GF}$ , thinking $SA(LN(Cat(i_t,b_t)))$ as $a_k\mu_k$ in Eq. \ref{eq:b_gf}.
The bottom left graph in Fig. \ref{fig:fegf} shows the structure of the proposed GICA block, in comparison with the original CA block shown on its right.
To save the computational cost of cross-attention and self-attention blocks, we also borrow the idea of neighborhood attention from NAT \cite{hassani2023neighborhood, hassani2022dilated} for designing the GICA block. 

After the scale-wise fused features, $\{q_t\}_{t=1}^4$, are calculated, we aggregate them with upsampling and attention-based concatenation as follows:
%\vspace{-1mm}
\begin{equation}
\tilde{q}_t=g_t(CPA[q_t,\tilde{q}_{t+1}];\theta_g^t),~~t=1,2,3,4.
	%\vspace{-1mm}
\end{equation}
Here, $CPA[\cdot, \cdot]$ refers to the concatenation operation with a channel and space attention layer, $g_1(\cdot;\theta_g^1)$ is a small convolutional network, and $g_t(\cdot;\theta_g^t),t=2,3,4$ denotes the upsample block illustrated in Fig. \ref{fig:fegf}. In addition, we define $\tilde{q}_{5}=[i_4,p_4]$ as the supplement to upsample $q_4$. Then the final output of the whole FeGF module is $q_{Fe}=\tilde{q}_1$.



With such a construction, our proposed GICA block has the capability to not only retain the effective properties of CA but also inherit the advantages of the GF mechanism. These properties can be preliminarily observed in Fig. \ref{fig:features},  which shows the outputs of mid-processes, including the output of the cross-attention module, $b_ts$, and $q_ts$. It can be seen that the outputs of CA mainly depict edge information, and $b_ts$ tends to preserve residual contents from filtering inputs, which show similar behaviors to the mechanism of GF.

\begin{figure}[t]
	\setlength{\abovecaptionskip}{0.2cm}
	\centering
	% \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
	\includegraphics[width=1\linewidth]{./results/features.pdf}
	%\vspace{-0.5cm}
	\caption{The visualization of middle features in ImGF (left) and FeGF (right).}
	\label{fig:features}
	\vspace{-0.5cm}
\end{figure}
% With such a construction, our FeGF-block not only can inherit the effectiveness of the cross-attention module but is also able to explicitly model guided image fusion and reconstruction tasks, making the overall structure better fit GF which has superior performance on these problems traditionally. 
% As discussed in Section \ref{sec:ca}, we introduce the cross-attention module for two reasons. For one thing, it has been proven effective in diverse information fusion tasks \cite{tan2019lxmert, zhang2022segmentation, chen2021crossvit}. For the other, as mentioned in Section \ref{sec:ca}, the mechanism of cross-attention has a similarity with the guided filter mechanism and can be explained in a guided filtering way. In short, the reason why we introduce the cross-attention mechanism lies not merely in its superior information-capturing ability compared to regular convolutional modules, abilities attributed to its large receptive field and long-range information modeling capability, but also in its containing the physical mechanism of guided filter, which is powerful in traditional guided image restoration.


\subsubsection{ImGF module for image-domain guided fusion \label{sec:imgf}}

The ImGF module is designed to fuse $I$ and $P$ in a guided filtering way for better detail preservation, sharing a similar idea as \cite{pan2019spatially, wu2018fgf}. Specifically, it produces the fusion result by:
% \vspace{-1mm}
\begin{equation}
	Q_{Im} =  A_{Im} \circ I + B_{Im}, \label{eq:10}
	\vspace{-1mm}
\end{equation}
where $A_{Im}$ and $B_{Im}$ should be inferred using networks with the information of $I$ and $P$. This is expected to retain the textual information of $I$ as much as possible according to the physical model of GF discussed in Section \ref{sec:gf}.

As discussed before, $A_{Im}$ should characterize the intrinsic correlations between $I$ and $P$, and thus it is natural to use the features extracted from them as the input of the inference network. Besides, according to Eq. (\ref{eq:a_gf}), the statistics of guidance $I$, i.e., variance, is adopted to normalize $A$ in GF, and therefore it is reasonable to also treat $I$ as input for inferring $A_{Im}$. Combining these two observations, we can use a small convolutional network to infer $A_{Im}$:
%\vspace{-1mm}
\begin{equation}
	A_{Im} = F_A(\{i_1,p_1,I\};\theta_A), \label{eq:imgf_a}
	%\vspace{-1mm}
\end{equation}
where $F_A(\cdot;\theta_A)$ is the inference network parameterized by $\theta_A$, and $(i_1,p_1)$ denotes features output by the first CFE (Coupled Feature Extraction) block in the MCFE module. Note that we only use the features with the same spatial size as $I$ and $P$ here, which makes the concatenation operation simpler.

According to Eq. (\ref{eq:b_gf}), the calculation for $B$ in GF is based on $A$, $P$ and $I$. Therefore, we can use $I$ and $P$, as well as $A_{Im}$, as the input to the inference network of $B_{Im}$:
%\vspace{-1mm}
\begin{equation}
	B_{Im} = F_B(\{A_{Im},P,I\};\theta_B), \label{eq:imgf_b}
	%\vspace{-1mm}
\end{equation}
where $F_B(\cdot;\theta_B)$ is a small convolutional network parameterized by $\theta_B$.

With the designing mechanism discussed above, the learnable guided fusion in the image domain can be achieved by ImGF, as shown in Fig. \ref{fig:features}.
{\color{red}  It should be also noticed that though our ImGF module shares a similar idea with SVLRM \cite{pan2019spatially} by making the parameters $A$ and $B$ of GF learnable, we have dug the GF mechanism further. For the GF mechanism technically considered in the image
domain, SVLRM directly treats $P$ and $I$ as inputs to simultaneously predict
$A$ and $B$ without distinguishing them for learning, while we more closely follow the GF mechanism by using different source information to learn $A$ and $B$ as listed in Eq.(\ref{eq:imgf_a}) and (\ref{eq:imgf_b}). In that, our ImGF module has a more powerful ability to depict emphasized information in both parameters and achieve superior performance.}


\begin{figure}[t]
	\setlength{\abovecaptionskip}{0.2cm}
	\centering
	% \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
	\includegraphics[width=1\linewidth]{./network/fegf_v3.pdf}
	%\vspace{-0.5cm}
	\caption{The overview of FeGF module. The details are introduced in Sec.\ref{sec:fegf}}
	\label{fig:fegf}
	\vspace{-0.5cm}
\end{figure}

==> sec_bak/4_exp.tex <==
\section{Applications and Experiments}
In this section, we apply the proposed GIRNet to various GIR tasks, including GDSR, MFIF, pan-sharpening, and guided LRIE, and conduct a series of experiments to verify its effectiveness. Additionally, we also provide ablations studies to analyze the effects of each component of GIRNet. 
% Given our goal of developing a unified model applicable to different GIR problems, we compare our methods with general techniques and specialized approaches tailored to each task. This experimental protocol aims to demonstrate the broad utility and efficacy of the proposed GIRNet framework across diverse GIR applications. The compared generalized methods, which have been proven effective and widely useful in guided image restoration tasks, consist of GF \cite{he2010guided, he2012guided}, FGF \cite{wu2018fgf}, SVLRM \cite{pan2019spatially}, DKN\cite{kim2021deformable}, CUNet\cite{deng2020cunet}, and DAGF\cite{zhong2021dagif}. The specialized methods and detailed experiment settings are introduced as follows.

\subsection{GIRNet for GDSR}
The GDSR task aims at restoring an HR depth map from an LR one under the guidance of an RGB image captured in the same scene. 
% This is a typical GIR problem, where the LR depth map $P \in \mathbb{R}^{h\times w \times 1}$ is the to-be-restored image, and the HR RGB image $I \in \mathbb{R}^{H\times W \times 3} $ is regarded as the guidance, where $h<H$ and $w<W$. For many deep learning methods, $P$ is generally pre-upsampled, e.g., by bicubic interpolation, to be with the same spatial size of $I$, and we follow this preprocessing way. Then the output should be a reconstructed depth map $Q_{out}\in \mathbb{R}^{H\times W \times 1}$. In this task, we train GIRNet in a supervised way with $L_1$ Loss for 200 epochs, and the initial learning rate is $1\times10^{-4}$ and {\color{red} reduces by 0.2 every 40 steps.}
% \textbf{The number of the base channel in our backbone network is 48.}

% \noindent \textit{a. Experimental Settings}

\noindent\textbf{Settings.}
Following previous settings \cite{he2021towards, zhao2022dct}, we take the first 1000 paired images of the NYU V2 dataset \cite{silberman2012indoor} as the train dataset and take the last 449 pairs as a test dataset. Besides, the trained model is also tested on the Middlebury dataset\cite{hirschmuller2007mid} and the Lu \cite{lu2014depth} dataset for evaluating its generalization abilities. All datasets are considered three SR scales, i.e., 4x, 8x, and 16x.
% For all datasets, we obtain low-resolution depth maps by downsampling the given high-resolution depth maps with the bicubic interpolation and consider three SR scales, i.e., 4x, 8x, and 16x.

To evaluate its strength, we compare our proposed GIRNet with 6 general-purpose GIR techniques, including the classical GF \cite{he2010guided, he2012guided}, and five deep learning-based methods, FGF \cite{wu2018fgf}, SVLRM \cite{pan2019spatially}, DKN\cite{kim2021deformable}, CUNet\cite{deng2020cunet}, and DAGF\cite{zhong2021dagif}.
Besides, we also compare four state-of-the-art specialized deep learning-based GDSR approaches, including FDSR \cite{he2021towards}, DCTNet\cite{zhao2022dct},  AHMF \cite{zhong2021high}, and SSDNet \cite{zhao2023spherical}. 
To enable quantitative comparison, we retrain all the general methods under the same setting as ours and utilize the widely adopted root-mean-square error (RMSE) as the metric to evaluate the performance of all compared methods across all GDSR datasets.

% \subsubsection{Competeting methods and evaluation metrics\label{sec:cm}}
% Since our developing goal is a unified model that can be applied to different GIR tasks, we will compare our methods with general-purpose GIR techniques and the methods designed for a specific task. Six representative general purpose methods are considered in all our experiments, including the classical GF \cite{he2010guided, he2012guided}, and five deep learning-based methods, FGF \cite{wu2018fgf}, SVLRM \cite{pan2019spatially}, DKN\cite{kim2021deformable}, CUNet\cite{deng2020cunet}, and DAGF\cite{zhong2021dagif}.
% For the GDSR task, we also compare four state-of-the-art specialized deep learning-based approaches, including FDSR \cite{he2021towards}, DCTNet\cite{zhao2022dct},  AHMF \cite{zhong2021high}, and SSDNet \cite{zhao2023spherical}. 
% To enable quantitative comparison, we utilize the widely adopted root-mean-square error (RMSE) as the metric to evaluate the performance of all compared methods across all GDSR datasets.

\noindent\textbf{Experimental Results.}
The quantitative results of all the competing methods across all datasets are summarized in Tabel \ref{tab:gdsr}. As can be seen from the table, our proposed approach GIRNet attains the leading performance across all benchmark datasets evaluated, indicating that our proposed method can reconstruct the depth map closest to the ground truth across different scenarios. Besides, considering the average result under each SR scale, our method also consistently performs the best, showing its robustness in handling the GDSR task with various degrees of degradation.

It can be seen from Fig.\ref{fig:gdsr} that our qualitative results are also promising. Compared with the methods that are implemented with image level-guided filtering mechanisms, including GF \cite{he2010guided}, FGF \cite{wu2018fgf}, and SVLRM \cite{pan2019spatially}, our method is able to avoid artifacts like ghosting and preserve structures {\color{red}simultaneously}. When competing against other general deep learning-based GIR approaches like FDKN\cite{kim2021deformable}, CUNet \cite{deng2020cunet}, and DAGF \cite{zhong2021dagif}, our method better reconstructs fine texture details. As for the specialized GDSR method, e.g. FDSR \cite{guo2018hierarchical}, AHMF\cite{zhong2021high}, DCTNet\cite{zhao2022dct}, SSDNet \cite{zhao2023spherical}, our method demonstrate superior performance through smooth surfaces and clear depiction of details. These observations show our method effectively overcomes generative methods' limitations of existing general-purpose GIR methods and even outperforms state-of-the-art deep models for the GDSR task.


\begin{figure*}[t]
	\centering
 \captionsetup[subfloat]{labelsep=none,format=plain,labelformat=empty}
	\setlength{\abovecaptionskip}{0.1cm}
	\subfloat[RGB ]{\includegraphics[width=0.14\linewidth]{./results/gdsr/color.pdf}}
	\subfloat[Bicubic (Lr) ]{ \includegraphics[width=0.14\linewidth]{./results/gdsr/lr.pdf}}
	\subfloat[GF]{ \includegraphics[width=0.14\linewidth]{./results/gdsr/GIF.pdf}} 
	\subfloat[FGF ]{	\includegraphics[width=0.14\linewidth]{./results/gdsr/FGF.pdf}}
	\subfloat[SVLRM ]{ \includegraphics[width=0.14\linewidth]{./results/gdsr/SVLRM.pdf}}
	\subfloat[FDKN]{	\includegraphics[width=0.14\linewidth]{./results/gdsr/FDKN.pdf}} 
 \subfloat[CUNet]{	\includegraphics[width=0.14\linewidth]{./results/gdsr/CUNet.pdf}} 
 \\
 % \vspace{-3mm}
 \subfloat[DAGF ]{	\includegraphics[width=0.14\linewidth]{./results/gdsr/DAGF.pdf}}
 \subfloat[FDSR]{	\includegraphics[width=0.14\linewidth]{./results/gdsr/FDSR.pdf}}
 \subfloat[AHMF ]{	\includegraphics[width=0.14\linewidth]{./results/gdsr/AHMF.pdf}}
 \subfloat[DCTNet ]{	\includegraphics[width=0.14\linewidth]{./results/gdsr/DCTNet.pdf}}
 \subfloat[SSDNet ]{	\includegraphics[width=0.14\linewidth]{./results/gdsr/SSDNet.pdf}}
 \subfloat[GIRNet]{	\includegraphics[width=0.14\linewidth]{./results/gdsr/GIRNet.pdf}}
  \subfloat[GT]{	\includegraphics[width=0.14\linewidth]{./results/gdsr/gt.pdf}}
	\caption{Visual comparison of competed methods on the 16x Middlebury dataset of the GDSR task. }
	\vspace{-0.5cm}
	\label{fig:gdsr} 
\end{figure*}

\begin{table}[!ht]
\tiny
\setlength\tabcolsep{3pt}
	\centering
	% \setlength{\abovecaptionskip}{0.1cm}
	\caption{Quantitative comparison with the generative and state-of-the-art methods on the GDSR task. We use the RMSE metric (The lower the better). The best performance is shown in bold, and the second is underlined. }
	\begin{tabular}{ccccccccccccc}
		\toprule
		\multirow{2}{*}{Methods}& \multicolumn{3}{c}{Middlebury} & \multicolumn{3}{c}{NYU V2} &  \multicolumn{3}{c}{Lu} & \multicolumn{3}{c}{Average}\\ 
		\cmidrule(lr){2-4}
            \cmidrule(lr){5-7}
            \cmidrule(lr){8-10}
            \cmidrule(lr){11-13}
		~ & 4x & 8x & 16x & 4x & 8x & 16x & 4x & 8x & 16x & 4x & 8x & 16x \\ \hline
 GF\cite{he2010guided}& 3.13 & 4.00 & 6.19 & 5.97 & 7.40 & 11.23 & 4.20 & 5.21 & 7.46 & 4.43  & 5.54  & 8.29   \\
        FGF \cite{wu2018fgf} & 1.36  & 2.28  & 4.34  & 2.39  & 3.82  & 6.98  & 1.37  & 2.35  & 4.61  & 1.71  & 2.82  & 5.31  \\ 
        SVLRM \cite{pan2019spatially} & 1.18 & 2.43 & 5.33 & 1.82 & 3.67 & 7.87 & 1.04 & 2.51 & 6.15 & 1.35  & 2.87  & 6.45   \\ 
        FDKN \cite{kim2021deformable} & 1.09  & 2.09  & 4.27  & 1.64  & 3.30  & 6.62  & \underline{0.79}  & 2.07  & 4.83  & 1.17  & 2.49  & 5.24 \\ 
        CUNet \cite{deng2020cunet}& 1.28 & 2.40 & 4.73 & 2.22 & 4.02 & 7.88 & 1.05 & 2.48 & 5.19 & 1.52  & 2.97  & 5.93   \\ 
        DAGF \cite{zhong2021dagif} & 1.28 & 2.66 & 3.80 & 2.66 & 4.97 & 7.19 & 1.26 & 2.60 & 4.77 & 1.73  & 3.41  & 5.25   \\ \hline
        FDSR \cite{he2021towards} & 1.06 & 2.08 & 4.17 & 1.78 & 3.17 & 5.94 & 1.15 & 2.19 & 5.08 & 1.33  & 2.48  & 5.06   \\ 
        AHMF \cite{zhong2021high} & 1.19 & 2.35 & 4.76 & 1.83 & 3.74 & 7.16 & 0.96 & 2.33 & 5.38 & 1.33  & 2.81  & 5.77   \\
        DCTNet \cite{zhao2022dct} & 1.10& 2.05 & 4.19 & 1.73& 3.56& 6.50 & 0.88& 1.85& 4.39 & 1.24 &2.49 &	5.03 \\ 
        SSDNet \cite{zhao2023spherical} & \underline{1.02} & \underline{1.91} & \underline{4.02} & \textbf{1.60} & \underline{3.14} & \underline{5.86} & 0.80 & \underline{1.82} & \underline{4.77} & \underline{1.14}  & \underline{2.29}  & \underline{4.88}   \\ \hline
        GIRNet (Ours) & \textbf{0.99} & \textbf{1.78} &\textbf{3.46}& \underline{1.63} & \textbf{3.10} & \textbf{5.85} & \textbf{0.74} &\textbf{1.73} & \textbf{4.55} & \textbf{1.12} & \textbf{2.20}  & \textbf{4.62}   \\ \hline
	\end{tabular}
	\label{tab:gdsr}
	% \vspace{-2mm}
\end{table}
% \begin{table*}[!ht]
% 	\centering
% 	% \setlength{\abovecaptionskip}{0.1cm}
% 	\caption{GDSR }
% 	\begin{tabular}[c]{*{13}{c}}
% 		\toprule
% 		\multirow{2}{*}{Methods}& \multicolumn{3}{c}{Middlebury} & \multicolumn{3}{c}{NYU V2} &  \multicolumn{3}{c}{Lu} &\multicolumn{3}{c}{RGBDD}\\ 
% 		\cmidrule(lr){2-4}
%             \cmidrule(lr){5-7}
%             \cmidrule(lr){8-10}
%             \cmidrule(lr){11-13}
% 		~ & x4 & 8x & 16x & x4 & 8x & 16x & x4 & 8x & 16x & x4 & 8x & 16x \\ \hline
% 		GF \cite{he2012guided} &3.24&4.36&6.79&5.84&7.86&12.41&4.18&5.34&8.02 \\
% 		FGF \cite{wu2018fgf} & 1.94&3.36&5.81&3.21&5.92&10.45&2.45&4.42&7.26  \\
%             SVLRM \cite{pan2019spatially}&1.18&2.43&5.33&1.82&3.67&7.87&1.04&2.51&6.15&1.24&2.19\\
% 		DKN \cite{kim2021deformable} &1.23 &2.12 &4.24 &1.62 &3.26 &6.51 &0.96 &2.16 &5.11 &1.30 &1.96 &3.42 \\ 
% 		CUNet \cite{deng2020cunet} &  1.28 &2.40 &4.33 &2.22 &4.02 &6.78 &1.05 &2.48 &4.99 &1.28 &2.13 &3.45\\ 
%             DAGF \cite{zhong2021dagif} &1.28 & 2.66 & 3.80 & 2.66 & 4.97& 7.19& 1.26& 2.60& 4.77&&& \\
%         \hline
%         DCTNet\cite{zhao2022dct} &1.19 &2.35 &4.76 &1.83 &3.74 &7.16 &0.96 & 2.33 &5.38 &1.23 &2.12 &3.63\\
%         GraphSR \cite{de2022graphsr}& 1.11&2.12 &4.43 &1.79 &3.17 &6.02 &0.92 &2.05 &5.15 &1.30 &1.83 &3.12\\
%         % MADUNet \cite{madunet} &1.15 &1.69 &3.23 &1.51 &3.02 &6.23 &0.90 &1.74 &3.86\\
% 		% NAFNet \cite{chen2022nafnet} & \underline{23.73}  & \underline{0.837}  & \underline{0.126}  & \underline{34.16}  & \underline{0.909}  & \textbf{0.059}  & 30.86  &  \underline{0.908}  & \underline{0.082}   \\
% 		\hline
% 		GIRNet (Ours) &\underline{}{1.13} & \textbf{1.99} &\textbf{4.03} &\textbf{1.57} &\textbf{2.96} &\textbf{5.66} &\textbf{0.86 }& \textbf{1.95}& \textbf{4.81}&1.21&1.92&3.18  \\ \hline
% 	\end{tabular}
% 	% \label{tab:fusion}
% 	% \vspace{-2mm}
% \end{table*}

\begin{table}[!ht]
\footnotesize
\setlength\tabcolsep{3pt}
	\centering
	% \setlength{\abovecaptionskip}{0.1cm}
	\caption{The average quantitative results on the WorldView-III dataset}

	\begin{tabular}{ccccccc}
         \toprule
		Methods & PSNR$\uparrow$  &SSIM$\uparrow$ & SAM$\downarrow$ & ERGAS$\downarrow$ & SCC$\uparrow$ & Q$\uparrow$\\ 
		\hline
		GF \cite{he2012guided} & 27.78 & 0.805 & 0.125 & 6.542 & 0.893 & 0.497  \\
		FGF \cite{wu2018fgf} & 32.49	&0.920	&0.086	&3.971	&0.947	&0.722\\
            SVLRM \cite{pan2019spatially}&32.99&0.944	&0.092	&3.572	&0.959	&0.755 \\
		DKN \cite{kim2021deformable} & 27.46 &0.742 & 0.107 & 6.861 & 0.841 & 0.418 \\ 
		CUNet \cite{deng2020cunet} & 32.46	&0.927	&0.101	&3.993	&0.949	&0.736\\ 
        DAGF \cite{zhong2021dagif} & 31.57 & 0.886&0.117&4.444&0.937&0.684\\
        % CDDFuse \cite{zhao2023cddfuse} \\
        \hline
      LAGConv \cite{jin2022lagconv} & \underline{37.12} & \underline{0.972}	& \underline{0.053}	& \underline{2.264}	& \underline{0.980} &	\underline{0.823}\\
      PANNet\cite{yang2017pannet} &32.47	&0.913	&0.097	&3.927	&0.951	&0.724\\
      GPPNN \cite{xu2021gppnn} & 35.55 &	0.962	&0.065	& 2.719 &	0.973	& 0.794\\
        MADUNet \cite{madunet} & \underline{37.12}	&0.971	&0.054	&2.267	&\textbf{0.981}	& \underline{0.823} \\
        % PGCU \cite{zhu2023probability} \\
            \hline
    GIRNet (Ours) & \textbf{37.30} &	\textbf{0.973}	&\textbf{0.052}	&\textbf{2.215}	&\textbf{0.981}	& \textbf{0.830} \\ \hline
	\end{tabular}
	\label{tab:pan}
	% \vspace{-2mm}
\end{table}


\begin{table}[!ht] \footnotesize
	\centering
	\setlength{\abovecaptionskip}{0.1cm}
	\caption{Quantitative comparison on the REALMFF and Lytro Dataset of MFIF task. The best performance is shown in bold, and the second is underlined.}
	\begin{tabular}{cccccc}
		\toprule
		\multirow{2}{*}{Methods}& \multicolumn{3}{c}{RealMFF} & \multicolumn{2}{c}{Lytro} \\ 
		\cmidrule(lr){2-4}
            \cmidrule(lr){5-6}
         ~ & PSNR$\uparrow$  &SSIM$\uparrow$ & LPIPS$\downarrow$ & Q$_{MI}$$\uparrow$ & Q$_{S}$$\uparrow$ \\
            \hline
		GF \cite{he2012guided} &31.88&  0.918 & 0.098 & 1.8262 & 0.8408 \\
		FGF \cite{wu2018fgf} & 37.34 & 0.967 & \textbf{0.008} & 1.8675 & 0.8507 \\
            SVLRM \cite{pan2019spatially}&36.79& 0.975 & 0.014 & 1.8873 & \underline{0.8521} \\
		DKN \cite{kim2021deformable} & 34.22& 0.942 & 0.080 & 1.3742 & 0.8386\\ 
		CUNet \cite{deng2020cunet} & \underline{38.68} & 0.975 & 0.011 &1.8614 & 0.8410 \\ 
            DAGF \cite{zhong2021dagif} & 37.69 & 0.975 & 0.015 & 1.8961 & 0.8414 \\
            % CDDFuse \cite{zhao2023cddfuse} \\
            \hline
		IFCNN \cite{liu2017multi} & 31.61 &0.914 & 0.034 & 1.5769 & 0.7874\\
            SMFUSE \cite{ma2021smfuse} &38.54 & \underline{0.977} & 0.019 & 1.8687 & 0.8404 \\
            % U2Fusion \cite{}\\
            U2Fusion \cite{xu2020fusiondn} & 35.76 &0.972 & 0.047 & 1.8734 & 0.8318 \\
            ZMFF \cite{hu2023zmff} &34.88 & 0.956 & 0.028 & \underline{1.8874} & 0.8365  \\
            \hline
            GIRNet (Ours) & \textbf{39.71}&	\textbf{0.986} & \underline{0.009} & \textbf{1.9160} & \textbf{0.8545} \\ \hline
	\end{tabular}
	\label{tab:mfif}
	% \vspace{-2mm}
\end{table}

\begin{figure*}[t]
	\setlength{\abovecaptionskip}{0.2cm}
	\centering
	% \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
	\includegraphics[width=1\linewidth]{./results/pan/4.pdf}
	%\vspace{-0.5cm}
	\caption{ Visual comparison of competed methods on the WorldView-\uppercase\expandafter{\romannumeral3} of the pan-sharpening task. The bottom row refers to the corresponding RMSE maps.}
	\label{fig:pan}
	\vspace{-0.5cm}
\end{figure*}



\subsection{GIRNet for pan-sharpening}
The pan-sharpening problem focuses on restoring an HRMS image from an LRMS image with the help of an HR pan image.
% , where $h<H$ and $w<W$ and the channel number $C$ is varied according to datasets, which is 8 in our experiments. Similar to GDSR, the LRMS image P can be first pre-upsampled with spatial size $H\times W$. In this application, we train our GIRNet in a supervised way with $L_1$ Loss for 3000 epochs. The initial learning rate is $1\times 10^{-4}$ and decreases as the training iterations increase.
% It should be mentioned that, as demonstrated by Deng et al. \cite{jin2022lagconv}, the introduction of multi-scale structures does not improve performance for the pan-sharpening task but tends to lead to a loss of detail because of the downsampling operations. Therefore, we only use the one-scale structure in the SMFE and FeGF modules for GIRNet in this task.

% \noindent \textit{a. Experimental Settings}

\noindent\textbf{Settings.}
We use the WorldView-\uppercase\expandafter{\romannumeral3} dataset \cite{deng2022machine} for training and testing.
% where the LRMS images have 8 channels and are generated by bicubic downsampling with scale 4.
% \subsubsection{Competeting Methods and evalutation metrics.}
Similar to the GDSR experiments, we consider both general-purpose GIR methods and specialized methods. Specifically, we compare our method with the same set of general-purpose methods mentioned before, and four methods that represent the state-of-the-art for the pan-sharpening task, including LAGConv \cite{jin2022lagconv}, PANNet \cite{yang2017pannet}, GPPNN \cite{xu2021gppnn}, and MADUNet \cite{madunet}.

To comprehensively evaluate the performance of each competing method, we adopt six quality assessment metrics in this task.  Among them, PSNR and SSIM are the widely used image quality assessment metrics; 
% Among them, the peak signal-to-noise ratio (PSNR) and structural similarity (SSIM) indices are commonly used image quality assessment metrics that measure pixel-level error and structural fidelity;
the spectral angle mapper (SAM) \cite{yuhas1992discrimination} assessed spectral similarity for hyperspectral images (HSIs) without regard to intensity scaling; the relative dimensionless global error in synthesis (ERGAS) and correlation coefficient (SCC) captured error magnitudes across spectral bands for HSIs; and the Q index \cite{vivone2014critical} evaluated image quality comprehensively. 

\noindent\textbf{Experimental Results.}
The quantitative results are shown in Table \ref{tab:pan}. It can be seen from the table that our proposed GIRNet ranks the best with respect to all the metrics, significantly outperforming the general-purpose GIR methods and also performing competitively against the state-of-the-art pan-sharpening methods. Specifically, GIRNet generates sharpened outputs with the highest PSNR and SSIM values in comparison to the  HRMS images, demonstrating its strong ability to preserve spatial information content. Besides, it also exhibits the lowest SAM and ERGAS values, indicating it most accurately retains the {\color{red} native original} spectral features and spatial patterns of the source data. Regarding SCC, GIRNet's best performance shows its effectiveness in maintaining local cross-band correlations. Furthermore, the leading score with respect to the full-reference Q index demonstrates its capacity to synthesize results most consistent with human perceptual judgments. All these quantitative results clearly verify the effectiveness of the proposed GIRNet in dealing with the pan-sharpening task.

% The qualitative results are shown in Fig.\ref{fig:pan}. With the help of Root Mean Square Error (RMSE) maps in the bottom row, it can be found that our methods have succeded in recovering the degraded details and shown outstanding performance compared with both of the generative methods and the specifically-designed pan-sharpening methods.
The qualitative results in Fig.\ref{fig:pan} provide a visual comparison of our proposed method against existing ones. As shown in the top row, our GIRNet is able to successfully reconstruct fine-scale details that were degraded in the LrMS images. The root mean square error (RMSE) maps in the bottom row provide a more easily observable validation of these qualitative findings. Specifically, the RMSE maps show that our method achieves the lowest error values, indicating its predictions most closely match the HRMS images. These results suggest our method can effectively leverage contextual information to reconstruct high-frequency details for this task.

\subsection{GIRNet for MFIF}
The MFIF task aims at fusing spatially complementary visual content
from multiple source frames exhibiting focus disparities and reconstructing an all-in-focus image. Typically in this task, two inputs depicting the same scene at near and far focal distances are fused. 
Therefore, this problem can be treated as a mutually guided image restoration, where the two input images guide each other for the final reconstruction. Besides, the MFIF task is commonly formulated in an unsupervised manner to meet practical requirements, and thus we implement our experiment along this setting.
The detailed network and training losses specifically modified for this task are shown in SM because of the space limitation.
% Since our proposed GIRNet distinguishes the guidance image from the guided image for two input sources, we need to slightly modify it to adapt to this task. 
% Specifically, we employ a dual-guidance framework, within which to operate in parallel and each GIRNet takes one image as the guidance and the other as the guided one.
% Then the middle results of the two GIRNet branches are fused at the output layer to get the final reconstruction.
% The whole dual framework is as follows:
% \begin{gather}
%     Q_{out}^1 = GIRNet_1(I_1, I_2),\\
%     Q_{out}^2 = GIRNet_2(I_2, I_1),\\
%     Q_{out} = Conv(Cat(Q_{out}^1, Q_{out}^2))
% \end{gather}
% where $I_1, I_2 \in \mathbb{R}^{H\times W\times3}$ refers to inputs captured with near and far views. Besides, as mentioned in Sec.\ref{sec:rlmff}, the MFIF task is commonly formulated in an unsupervised manner to meet practical requirements, and thus we utilize two unsupervised losses for network training without relying on ground truth images:
% \begin{gather}
%     L_2 = s_1\|Q_{out}-I_1\|_2^2 + s_{2}\|Q_{out}-I_2\|_2^2,\\
%     L_{grad} = s_{1}\|\nabla Q_{out}-\nabla I_1\|_2^2 + s_{2}\|\nabla Q_{out}-\nabla I_2\|_2^2,\\
%     L = L_2 + L_{grad},
% \end{gather}
%  {\color{red} where $s_{1} = sgn(HF(I_1)-min(HF(I_1), HF(I_2)))$, $s_{2} = 1 - s_{1}$. $\nabla$ refers to the gradient operator. $HF(\cdot)$ refers to the high-frequency contents of the image, calculated by the Gaussian filtering kernel.} In the MFIF application, we train the GIRNet for 200 epochs whose batch size is 16 and the initial learning rate is $1x10^{-4}$.

% \noindent \textit{a. Experimental Settings}
\noindent\textbf{Settings.}
We evaluate the effectiveness of our method on the Real-MFF dataset \cite{zhang2020real}, which consists of various natural multi-focus images with ground truth, generated by light field images.
We use the first 650 pairs of images for training and the last 60 pairs of images for testing. 
Besides, we conduct an evaluation on the widely used real-world Lytro dataset \cite{nejati2015multi} to show our generalization. 
% It contains 20 pairs of multi-focus images obtained by the light-field camera with a size of 520 × 520.
% It is worth noting that obtaining ground truth images for reference is challenging to achieve in practice. As such, our proposed model is trained in an unsupervised fashion, without directly supervised learning from fused ground truths.

% \subsubsection{Competeting Methods and evaluation metrics}
For comparison, in addition to the six general-purpose GIR methods used before, four state-of-the-art DL-based MFIF methods were adopted for evaluation, including IFCNN \cite{liu2017multi}, SMFUSE \cite{ma2021smfuse}, U2Fusion \cite{xu2020fusiondn}, and ZMFF \cite{hu2023zmff}. All the competing methods are trained in an unsupervised manner or implemented in a zero-shot way, without reference to the ground truth.
To numerically evaluate the fusion results, we adopt three common image quality assessment metrics, including PSNR, SSIM, and LPIPS.  Among these metrics, PSNR and SSIM are general image quality assessment metrics, LPIPS is a deep feature-based metric aiming at assessing the perceptual quality of an image with a reference image.
For evaluation on the non-reference dataset Lytro, we use the information theory-based metrics Q$_{MI}$ and the image structure similarity-based metric Q$_{S}$ following \cite{hu2023zmff}.

\noindent\textbf{Experimental Results.}
The qualitative results of all competing methods are reported in Table \ref{tab:mfif}, and we can see that our GIRNet achieves the best performance among all methods, obtaining 1.03 dB improvement in PSNR and 0.009 improvement in SSIM compared with the second best ones, and takes the second place on LPIPS, showing our outstanding perceptual quality.
For the Lytro dataset, we also achieve the first place among all methods, presenting that our results have the richest information extracted from source images and share the highest similarity with sources based on SSIM.
These improvements demonstrate the effectiveness of our method for this task. 

% The qualitative results are shown in Fig.\ref{fig:mff}. From the bottom row, we can see that our methods succeed in combining both near and far views. We also show error maps which refer to the mean square error (MSE) distance between prediction and ground truth. The error maps show that our method can recover more accurate structures compared with both generative and specific methods even in an unsupervised way. 
The visual results presented in Fig.\ref{fig:mff} further verify the superiority of the proposed GIRNet over existing methods. Specifically, as shown in the top row, our method is able to successfully synthesize images that integrate both near-view details and far-view context. The mean square error (MSE) maps in the bottom row make this observation clearer and indicate a more accurate structural reconstruction of our method against other competing methods, with reference to the ground truth. The visual comparisons of Lytro are shown in the SM because of the space limitation.
% In comparison to both generative models and techniques designed specifically for multi-focus fusion, our method qualitatively synthesizes better-focused images and quantitatively achieves superior performance.

\begin{figure*}[t]
	\setlength{\abovecaptionskip}{0.2cm}
	\centering
	% \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
	\includegraphics[width=1\linewidth]{./results/mfif/mff_709_2.pdf}
	%\vspace{-0.5cm}
	\caption{Visual comparison of competed methods on the Real-MFF dataset of the MFIF task. The bottom row refers to the corresponding error maps.}
	\label{fig:mff}
	% \vspace{-0.5cm}
\end{figure*}


% \begin{figure*}[t]
% 	\centering
%  \captionsetup[subfloat]{labelsep=none,format=plain,labelformat=empty}
% 	\setlength{\abovecaptionskip}{0.1cm}
% 	\subfloat[RAW ]{\includegraphics[width=0.14\linewidth]{./results/lrie/inp.pdf}}
% 	\subfloat[Bicubic ]{ \includegraphics[width=0.14\linewidth]{./results/lrie/bi.pdf}}
% 	\subfloat[GF]{ \includegraphics[width=0.14\linewidth]{./results/lrie/gf.pdf}} 
% 	\subfloat[FGF ]{	\includegraphics[width=0.14\linewidth]{./results/lrie/fgf.pdf}}
% 	\subfloat[SVLRM ]{ \includegraphics[width=0.14\linewidth]{./results/lrie/svlrm.pdf}}
% 	\subfloat[FDKN]{	\includegraphics[width=0.14\linewidth]{./results/lrie/fdkn.pdf}} 
%  \subfloat[CUNet \cite{deng2020cunet}]{	\includegraphics[width=0.14\linewidth]{./results/lrie/fdkn.pdf}} 
%  \\
%  \vspace{-3mm}
%  \subfloat[DAGF ]{	\includegraphics[width=0.14\linewidth]{./results/lrie/dagf.pdf}}
%  \subfloat[SID]{	\includegraphics[width=0.14\linewidth]{./results/lrie/sid.pdf}}
%  \subfloat[SGN]{	\includegraphics[width=0.14\linewidth]{./results/lrie/sgn.pdf}}
%  \subfloat[EEMEFN]{	\includegraphics[width=0.14\linewidth]{./results/lrie/eemefn.pdf}}
%  \subfloat[DBLE]{	\includegraphics[width=0.14\linewidth]{./results/lrie/dble.pdf}}
%  \subfloat[GIRNet]{	\includegraphics[width=0.14\linewidth]{./results/lrie/girnet.pdf}}
%   \subfloat[GT]{	\includegraphics[width=0.14\linewidth]{./results/lrie/gt.pdf}}
% 	\caption{Visual comparison of competed methods on the SID-Sony dataset of the LRIE task.}
% 	\vspace{-0.5cm}
% 	\label{fig:lrie} 
% \end{figure*}


\subsection{GIRNet for guided LRIE}
% The goal of LRIE is to enhance the quality of the RAW image captured under extremely low-light conditions, typically through the deep image signal processing (ISP) pipeline \cite{chen2018learning}. Currently, a widely used and effective strategy for dealing with this task is to make use of guide information, either self-generated \cite{zhu2020eemefn} or auxiliary \cite{dong2022abandoning}. Therefore, our GIRNet can be naturally applied to the LRIE task, by treating it as a  GIR problem. To distinguish whether the guidance is self-generated or auxiliary, we consider two sets of applications here. The first is pure LIRE, i.e., one can only use the information of the RAW image itself, which means that the guidance can only be self-generated; the second is the guided LIRE, in which one can use auxiliary guidance information, e.g., the red flashlight image \cite{lamba2021red} or the monochrome image \cite{dong2022abandoning}.


Following the work by Xiong et al. \cite{xiong2021mffnet} and Dong et al. \cite{dong2022abandoning}, which respectively used the red flashlight image and the monochrome image as the guidance for low-light image enhancement of RAW image, we consider two scenarios of guided low-light image enhancement tasks: (1) RAW image with red flashlight RAW guidance and (2) RAW image with monochrome RAW guidance. 

% \subsubsection{Datasets}
\noindent\textbf{Settings.}
For the first task, we synthesize paired RAW/red flashlight dataset from the Sony dataset of the SID dataset \cite{chen2018learning}, which is constructed by extremely low-light RAW images.
% Images in the Sony dataset are captured by the Sony $\alpha$7S \uppercase\expandafter{\romannumeral2} Bayer sensor with the size $4256 \times 2848 \times 1$.
 For the second, we adopt the Mono-Colored RAW (MCR) paired dataset collected by Dong et al. \cite{dong2022abandoning}. 
 % All the input RAW images are packed into 4 channels before being inputted into networks following \cite{chen2018learning}.
% \subsubsection{Competing methods and evaluation metrics} 

For comparison, in addition to the six general-purpose GIR methods, we consider two recently proposed guided LRIE methods, i.e., MFFNet \cite{xiong2021mffnet} and DBLE \cite{dong2022abandoning}.
Four metrics, including PSNR, SSIM, LPIPS \cite{zhang2018lpips} and Delta E ($\triangle E^{*}$) \cite{backhaus2011color}, are adopted for quantitative evaluation, where
% Among these metrics, PSNR and SSIM are general image quality assessment metrics, LPIPS is a deep feature-based %\footnote{We employ the AlexNet as the feature extractor.} 
% metric aiming at assessing the perceptual quality of an image with a reference image, and 
$\triangle E^{*}$ is a metric to measure the color distortion.

% \subsubsection{ Experimental Results}
\noindent\textbf{Experimental Results.}
The quantitative evaluation results for all comparison methods are reported in Table \ref{tab:glrie}. It can be seen that our proposed GIRNet model achieves superior performance across all evaluated metrics compared with other competing approaches, which shows the outstanding abilities of our method in reconstructing textual and contextual information and overcoming color biases.

{\color{red} Fig. \ref{fig:red}-\ref{fig:mcr} show example qualitative results as well as the corresponding error maps. It can be visually observed from the error maps that our method produces results with fewer residuals compared with the ground truths.}

% As demonstrated in the error maps for images corrupted with both noise and color casts, GIRNet restores images with finer edges and more accurate textures. This validates the robustness of our approach against common image artifacts like noise and color distortions.

 
% \begin{table}[!ht]
% 	\small
% 	\centering
%  \setlength{\abovecaptionskip}{0.0cm}
% 	\caption{Quantitative results of all competing LRIE methods on the SID dataset. The best and second-best results are highlighted in bold and with an underline, respectively.\label{tab:sid} }
% 	\begin{tabular}{ccccc}
% 		\toprule
% 		Methods & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ &$\triangle \textit{E}^{*}\downarrow$ \\ \hline
% 		GF \cite{he2010guided}   & 16.03 & 0.519 & 0.410  & 18.76        \\
% 		FGF \cite{wu2018fgf}   & 28.84 & 0.768 & 0.310 & 5.035    \\
%             SVLRM \cite{pan2019spatially} &28.56 & 0.763 & 0.260 & 5.587  \\
%             DKN \cite{kim2021deformable} & 25.39 & 0.692&0.362&6.848 \\
%             CUNET \cite{deng2020cunet} & 28.37& 0.774 & 0.280 & 5.579 \\
%              DAGF \cite{zhong2021dagif} & 30.07&	0.800 &	0.245 &	4.500 \\
%              % CDDFuse \cite{zhao2023cddfuse} \\
%             \hline
% 		SID \cite{chen2018learning}     & 29.57 & 0.799 & \underline{0.246} & 4.901      \\
%         % LRDE \cite{xu2020lrde}  & 29.66 & 0.794 & 0.253  & 4.689 \\
% 		SGN  \cite{gu2019sgn} & 29.45 & 0.796 & 0.248 & 4.936    \\
% 		EEMEFN \cite{zhu2020eemefn}   & \underline{30.08} & \underline{0.801} & 0.247 & \underline{4.662}    \\
% 		% RED \cite{lamba2021red}    & 28.66 & 0.790  & 0.312 & 20.17   \\
% 		DBLE \cite{dong2022abandoning} & 29.70 & 0.796 & 0.247 & 4.759      \\
       
%         % DNF \cite{jin2023dnf} &28.71 &  0.726  & 0.391 & &30.62&0.797&0.343 & & 2.800 & 57.00\\
%         \hline
%   GIRNet (Ours)   & \textbf{30.27} & \textbf{0.804} &\textbf{0.245} & \textbf{4.522}   \\\hline
% 	\end{tabular}
% 	\vspace{-4mm}
% \end{table}


\begin{table}[!ht]\tiny
\setlength\tabcolsep{3pt}
	\centering
	\setlength{\abovecaptionskip}{0.1cm}
	\caption{Quantitative results of all competing methods on guided LIRE tasks. The best and second-best results are highlighted in bold and with an underline, respectively.}
	\begin{tabular}{ccccccccc}
		\toprule
		\multirow{2}{*}{Methods}&  \multicolumn{4}{c}{Sony (RAW+Red)} &  \multicolumn{4}{c}{MCR (RAW+Mono)} \\ 
  % \multirow{2}{*}{Methods}& \multicolumn{3}{c}{Middlebury} & \multicolumn{3}{c}{NYU V2} &  \multicolumn{3}{c}{Lu} & \multicolumn{3}{c}{Average}
            \cmidrule(lr){2-5}
            \cmidrule(lr){6-9}
		% \hline
		~ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & $\triangle E^{*}\downarrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & $\triangle E^{*}\downarrow$   \\ \hline
		GF \cite{he2012guided} & 16.25 & 0.674 & 0.328 & 18.61 & 16.04 & 0.697 & 0.405 & 14.47  \\
		FGF \cite{wu2018fgf}  & 30.80  & 0.857  & 0.129  & 4.453 & 23.93  & 0.830  & 0.176 & 6.660  \\
            SVLRM \cite{pan2019spatially}&32.34 & 0.890 & 0.075 & 3.857 & 25.83	& 0.879& 0.103 & 5.758 \\
		DKN \cite{kim2021deformable} & 26.68  & 0.720  & 0.232 & 6.467 & 23.43  & 0.838  & 0.151  & 7.528 \\ 
		CUNet \cite{deng2020cunet} & 30.99  & 0.881  & 0.091 & 4.290 & 19.70  & 0.673  &  0.257 & 11.55 \\ 
            DAGF \cite{zhong2021dagif} & 27.96 &0.887 &0.090 & 5.592 & 26.67 &0.873&0.126&5.241\\
            % CDDFuse \cite{zhao2023cddfuse} \\
		\hline
		DBLE \cite{dong2022abandoning}  & \underline{33.36}  & \underline{0.893} & \underline{0.075}  & \underline{3.622} & \underline{31.69}  & \underline{0.908}  & \underline{0.082} &\underline{3.133}  \\ 
		MFFNet \cite{xiong2021mffnet}  & 30.99  & 0.876  & 0.101 & 4.440 & 28.62  & 0.902  & 0.096 & 4.316  \\
		% NAFNet \cite{chen2022nafnet} & \underline{23.73}  & \underline{0.837}  & \underline{0.126}  & \underline{34.16}  & \underline{0.909}  & \textbf{0.059}  & 30.86  &  \underline{0.908}  & \underline{0.082}   \\
		\hline
		GIRNet (Ours) &\textbf{34.25}  & \textbf{0.902}  & \textbf{0.067} & \textbf{3.304} & \textbf{32.11} 	&\textbf{0.925} &	\textbf{0.065} &	\textbf{3.077 }  \\ \hline
	\end{tabular}
	\label{tab:glrie}
	\vspace{-2mm}
\end{table}


\begin{figure*}[t]
	\setlength{\abovecaptionskip}{0.2cm}
	\centering
	% \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
	\includegraphics[width=1\linewidth]{./results/red/10003.pdf}
	%\vspace{-0.5cm}
	\caption{Visual comparison of competed methods on the SID-Sony dataset of the red-guided LRIE task. The bottom row refers to the corresponding error maps.}
	\label{fig:red}
	% \vspace{-0.5cm}
\end{figure*}

\begin{figure*}[t]
	\setlength{\abovecaptionskip}{0.2cm}
	\centering
	% \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
	\includegraphics[width=1\linewidth]{./results/mcr/mcr_48.pdf}
	%\vspace{-0.5cm}
	\caption{ Visual comparison of competed methods on the MCR dataset of the mono-guided LRIE task. The bottom row refers to the corresponding error maps.}
	\label{fig:mcr}
	% \vspace{-0.5cm}
\end{figure*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure*}[t]
	\setlength{\abovecaptionskip}{0.2cm}
	\centering
	% \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
	\includegraphics[width=1\linewidth]{./results/ablation.pdf}
	%\vspace{-0.5cm}
	\caption{ Visual comparison of competed methods on the MCR dataset of the mono-guided LRIE task. The bottom row refers to the corresponding error maps.}
	\label{fig:ablation}
	% \vspace{-0.5cm}
\end{figure*}
\begin{table}[t]
\setlength\tabcolsep{3pt}
\footnotesize
	\centering
	% \setlength{\abovecaptionskip}
	\caption{RMSE results of \textbf{ablation study} on the 16x GDSR task.\label{tab:ablation} }
	% \begin{adjustbox}{width=0.95\linewidth, center}
		\begin{tabular}{l cccc}
			 \toprule
			Settings & Middlebury &NYU V2 &Lu &Average \\ \hline
                (a) SMFE$_p$   &  3.53 &5.89 &4.57& 	4.63  \\ 
                (b) SMFE$_s$  & 3.61 & 6.10 &4.45 &4.75 \\
                \hline
                (c) only FeGF (w/o ImGF)  &3.54 &	5.95 	&4.48 & 4.66 \\ 
                (d) ImGF $\rightarrow$ Conv & 3.52 	& 5.89 &4.53 & 4.65 \\
                (e) SVLRM & 5.33 & 7.87 & 6.15 & 6.45\\
                (f) SVLRM with ImGF & 4.79 & 7.28 & 5.57 & 5.88 \\
                \hline
                (g) only ImGF (w/o FeGF) & 6.36 & 11.2 &7.22 & 7.35 \\
                 (h) FeGF $\rightarrow$ CNN &3.63 	& 6.11 	&4.62 	& 4.79 \\
                 (i) GICA $\rightarrow$ Conv+GF & 3.48 &	6.12 & 4.29 & 4.74 \\
                 (j) GICA $\rightarrow$ CA & 3.70 &	6.28 & 4.63 & 4.87 \\

                 
                  % ImGF $\rightarrow$ SVLRM \\
			% only ImGF$_{l}$ & & & & & 0.076 & 18.97 \\ 
			\hline
			(k) GIRNet (Ours) & \textbf{3.38} &	\textbf{5.75} 	& \textbf{4.38} & \textbf{4.57 }\\\hline
		\end{tabular}
	% \end{adjustbox}
	% \vspace{-7mm}
\end{table}

 \subsection{Effectiveness of modules in GIRNet \label{sec:ablation}}
In this subsection, we conduct experiments on the 16x GDSR task to verify the necessity and effectiveness of key modules, including SMFE, ImGF, and FeGF in the proposed GIRNet. The overall results are summarized in Tabel \ref{tab:ablation}, and shown in Fig. \ref{fig:ablation}. 



\begin{figure}[t]
	\setlength{\abovecaptionskip}{0.2cm}
	\centering
	% \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
	\includegraphics[width=1\linewidth]{./results/q_im_q_fe.pdf}
	%\vspace{-0.5cm}
	\caption{ Visual comparison of competed methods on the MCR dataset of the mono-guided LRIE task. The bottom row refers to the corresponding error maps.}
	\label{fig:abqq}
	% \vspace{-0.5cm}
\end{figure}


\noindent\textbf{Effectiveness of the SMFE module.}
% We conduct experiments to verify the necessity of the two key modules, ImGF and FeGF, in our GIRNet. These two modules are responsible for fusion in image and feature domains, respectively, and we show that both of them play important roles.
We first conduct ablation experiments to evaluate the effectiveness of our proposed SMFE module in cooperatively extracting shared and private information from source images. Specifically, we compared our model against two baselines\textemdash a \textbf{shared} setting where source images are directly concatenated as input, which is denoted as \textit{SMFE$_{s}$},  and a \textbf{private} setting where each source is processed independently by separate feature extractors, which is denoted as \textit{SMFE$_{p}$}.
For the shared baseline, the concatenated inputs were passed through a feature extractor with NAF blocks as the basic module, retaining the skip connections. In the private setting, each source was processed individually by isolated NAF feature extractors.

As shown in Table \ref{tab:ablation}, both settings exhibited decreased performance quantitatively compared to our full model across all datasets.
Qualitatively, visualization of results in Fig. \ref{fig:ablation} revealed that our SMFE module was able to better capture fine-grained details like object edges and produce images with a more even appearance, while the compared settings exhibited degraded ability in edge refinement and surface reconstruction. 
Furthermore, we visualize the extracted features by different approaches in Fig. \ref{fig:absmfe}. It can be observed that, compared with GIRNet, both the $i_ts$ and $p_ts$ of \textit{SMFE$_{p}$}, which are extracted respectively,  are unable to extract the necessary structural contents without the Mutual information extraction. In contrast, employing a completely shared SMFE to extract $i_{ts}$ and $p_{ts}$ preserves similar structural information across the two representations while also retaining unexpected texture details. 
% This evaluation empirically validates the effectiveness of our proposed module in disentangling shared and private representations from multiple related inputs, outperforming alternative designs that do not separate modality-specific information. It demonstrates the importance of modeling both shared and private content for the task of multi-modal image fusion.

\noindent\textbf{Effectiveness of the FeGF module.}
We began by investigating a model utilizing only the ImGF module to demonstrate the importance of the FeGF module. Not surprisingly, without feature restoration capabilities, the performance degraded substantially as shown in (g) Fig.\ref{fig:ablation} and Table \ref{tab:ablation}.
Additionally, to further evaluate the impact of incorporating the GF mechanism, we conducted an ablation experiment by completely replacing the whole FeGF module with a series of CNN layers. The results are reported quantitatively in Table \ref{tab:ablation} (h) and qualitatively depicted in Figure \ref{fig:ablation} (h), and both of them indicate performance degradation with respect to the full GIRNet model, validating the importance of the GF mechanism.
For deeper insight, we visualize the feature domain restoration output \textit{Q$_{Fe}$} with and without GF in Figure \ref{fig:abqq} (k) and (h). The reconstruction exhibits unclear edges when GF cues are not provided to guide the restoration, highlighting the role of the GF mechanism in preserving structures from the guidance features $i_ts$.

Since the GF mechanism is achieved in our model via the proposed GICA block, we want to further analyze its necessity. In specific, we conduct another ablation test of replacing the CA and SA blocks with standard CNN layers while maintaining the overall GF design. This setting keeps the GF mechanism by $q_t = A_t * i_t + b_t$, where $A_t$ and $b_t$ are learned by convolutional layers.
It can be seen from Table \ref{tab:ablation} that the quantitative performance is dropped by this setting. In addition, Fig. \ref{fig:abqq} and \ref{fig:ablation} (i) provide the visual results. It can be observed that the details are less clear compared with GIRNet due to the abilities of SA and CA to capture long-range dependencies, which is beneficial for reconstructing information degraded by downsampling operations.
When comparing (h) and (i), it can be seen that completely lacking the guidance of GF by completely replacing the FeGF module with ordinary CNN layers without the GF mechanism, can result in blurrier edges. All the observations indicate that the effectiveness of our FeGF module is not only from the attention blocks but also from the introduction of the GF mechanism which helps to preserve structural information from guidance features. 
Besides, we conduct the experiment of replacing our GICA block with the original CA block. It can be seen from (j) in Table \ref{tab:ablation} and Figure \ref{tab:ablation} that both the qualitative and quantitive results are degraded. Furthermore, when compared with (i), the original CA block performs worse, since it loses the important GF mechanism without the learned residual $b$ in Eq. \ref{eq:fegf_ca}.
Combined with quantitative findings, these provide preliminary evidence that both the FeGF module and its GF-based cross-attention modules contribute favorable information fusion beyond conventional CNN designs lacking these capabilities.

\noindent\textbf{Effectiveness of the ImGF module.}
To evaluate the effectiveness of ImGF, we first conduct an experiment without it and keep only the FeGF module.
As shown in (c) of Table \ref{tab:ablation}, removing ImGF led to degraded quantitative performance on all datasets. Qualitative results in (c) Fig.\ref{fig:ablation} further revealed deficits in this setting, that it loses fine image details and generates blurred edges. This validates that ImGF plays a crucial role in preserving the original textural information from the source images.

To further verify the effectiveness of the introduction of the GF mechanism in the ImGF module, we also conduct an experiment by replacing the ImGF module with CNN layers and observe the degraded performance both quantitatively and visually. Specifically, Fig.\ref{fig:ablation} (d) shows that the edges detected by the CNN-only model appear {\color{red}more blurry} compared to the present ImGF model. The output $Q_{Im}$ of this branch in this setting is shown in Fig. \ref{fig:abqq} (d). It can be observed that without the GF mechanism, the fused result \textit{Q$_{Im}$} suffers from loss of textual information and generates blurry edges. 
These results demonstrate that incorporating the GF into the ImGF module enhances model performance over using CNN layers alone.

{\color{red} As demonstrated in Section \ref{sec:imgf}, our proposed guided restoration module in the image domain follows more closely to the original GF mechanism compared with SVLRM \cite{pan2019spatially}. To show our effectiveness, we additionally conducted the experiment on SVLRM by replacing the inputs of its parameters learning network with our strategy. The compared quantitative results are listed in (e) and (f) in Table \ref{tab:ablation}. It can be observed that our mechanism have benefit in improving recovery performance. }

==> sec_bak/5_conclusion.tex <==
\section{Conclusion}

Though traditional joint filters and their inspired DNN methods have achieved outstanding performance on GIR tasks, the restoration images still suffer from unsatisfied performance with over-transferred artifacts or loss of details.
% Thus it's important to further explore the correlation between filtering mechanisms and DNNs for better fusion outputs.
To mitigate these problems, in this paper, we propose an effective GIRNet for the GIR tasks. In the image domain, we learn the parameters of GF with DNNs for the image-level fusion of sources. Furthermore, we deeply explore the correlation between the principles of GF and the CA module and propose a GICA block, where the CA module is specifically adapted for the GIR tasks according to GF, to construct the feature-level fusion sub-network. 
Experiments on the GIR tasks, including GDSR, MFIF, pansharpening, and guided LRIE,
have verified the effectiveness and wide applicability of the pro-
posed GIRNet. 
